Interim report for the International Muon Collider Collaboration (IMCC)

The International Muon Collider Collaboration (IMCC) [1] was established in 2020 following the recommendations of the European Strategy for Particle Physics (ESPP) and the implementation of the European Strategy for Particle Physics-Accelerator R&D Roadmap by the Laboratory Directors Group [2], hereinafter referred to as the the European LDG roadmap. The Muon Collider Study (MuC) covers the accelerator complex, detectors and physics for a future muon collider. In 2023, European Commission support was obtained for a design study of a muon collider (MuCol) [3]. This project started on 1st March 2023, with work-packages aligned with the overall muon collider studies. In preparation of and during the 2021-22 U.S. Snowmass process, the muon collider project parameters, technical studies and physics performance studies were performed and presented in great detail. Recently, the P5 panel [4] in the U.S. recommended a muon collider R&D, proposed to join the IMCC and envisages that the U.S. should prepare to host a muon collider, calling this their "muon shot". In the past, the U.S. Muon Accelerator Programme (MAP) [5] has been instrumental in studies of concepts and technologies for a muon collider.

==> AddAuthors/AddAuthors_old.tex <==
\newpage 
\thispagestyle{empty}

\vskip 10cm
\begin{center}
{\huge\bfseries
Interim report for the \\
International Muon Collider Collaboration (IMCC) }

\end{center}

\vspace{5mm}
{\small
\noindent
C.~Accettura$^{1}$, S.~Adrian$^{2}$, R.~Agarwal$^{3}$, C.~Ahdida$^{1}$, C.~Aim\'e$^{4}$, A.~Aksoy$^{1, 5}$, G.~L.~Alberghi$^{6}$, S.~Alden$^{7}$, N.~Amapane$^{8, 9}$, D.~Amorim$^{1}$, P.~Andreetto$^{10}$, F.~Anulli$^{11}$, R.~Appleby$^{12}$, A.~Apresyan$^{13}$, P.~Asadi$^{14}$, M.~Attia Mahmoud$^{15}$, B.~Auchmann$^{16, 1}$, J.~Back$^{17}$, A.~Badea$^{18}$, K.~J.~Bae$^{19}$, E.~J.~Bahng$^{20}$, L.~Balconi$^{21, 22}$, F.~Balli$^{23}$, L.~Bandiera$^{24}$, C.~Barbagallo$^{1}$, R.~Barlow$^{25}$, C.~Bartoli$^{26}$, N.~Bartosik$^{9}$, E.~Barzi$^{13}$, F.~Batsch$^{1}$, M.~Bauce$^{11}$, M.~Begel$^{27}$, J.~S.~Berg$^{27}$, A.~Bersani$^{28}$, A.~Bertarelli$^{1}$, F.~Bertinelli$^{1}$, A.~Bertolin$^{10}$, P.~Bhat$^{13}$, C.~Bianchi$^{26}$, M.~Bianco$^{1}$, W.~Bishop$^{17, 29}$, K.~Black$^{30}$, F.~Boattini$^{1}$, A.~Bogacz$^{31}$, M.~Bonesini$^{32}$, B.~Bordini$^{1}$, P.~Borges de Sousa$^{1}$, S.~Bottaro$^{33}$, L.~Bottura$^{1}$, S.~Boyd$^{17}$, M.~Breschi$^{26, 6}$, F.~Broggi$^{22}$, M.~Brunoldi$^{34, 4}$, X.~Buffat$^{1}$, L.~Buonincontri$^{35, 10}$, P.~N.~Burrows$^{36}$, G.~C.~Burt$^{37, 38}$, D.~Buttazzo$^{39}$, B.~Caiffi$^{28}$, S.~Calatroni$^{1}$, M.~Calviani$^{1}$, S.~Calzaferri$^{34}$, D.~Calzolari$^{1}$, C.~Cantone$^{40}$, R.~Capdevilla$^{13}$, C.~Carli$^{1}$, C.~Carrelli$^{41}$, F.~Casaburo$^{42, 11, 28}$, M.~Casarsa$^{43}$, L.~Castelli$^{42, 11}$, M.~G.~Catanesi$^{44}$, L.~Cavallucci$^{26, 6}$, G.~Cavoto$^{42, 11}$, F.~G.~Celiberto$^{45}$, L.~Celona$^{46}$, A.~Cemmi$^{41}$, S.~Ceravolo$^{40}$, A.~Cerri$^{47, 48, 39}$, F.~Cerutti$^{1}$, G.~Cesarini$^{40}$, C.~Cesarotti$^{49}$, A.~Chanc\'e$^{23}$, N.~Charitonidis$^{1}$, M.~Chiesa$^{4}$, P.~Chiggiato$^{1}$, V.~L.~Ciccarella$^{40, 42}$, P.~Cioli Puviani$^{50}$, A.~Colaleo$^{51, 44}$, F.~Colao$^{41}$, F.~Collamati$^{11}$, M.~Costa$^{52}$, N.~Craig$^{53}$, D.~Curtin$^{54}$, L.~D'Angelo$^{55}$, G.~Da Molin$^{56}$, H.~Damerau$^{1}$, S.~Dasu$^{30}$, J.~de Blas$^{57}$, S.~De Curtis$^{58}$, H.~De Gersem$^{55}$, T.~Del Moro$^{42, 41}$, J.-P.~Delahaye$^{1}$, D.~Denisov$^{27}$, H.~Denizli$^{59}$, R.~Dermisek$^{60}$, P.~Desir\'e Valdor$^{1}$, C.~Desponds$^{1}$, L.~Di Luzio$^{10}$, E.~Di Meco$^{40}$, K.~F.~Di Petrillo$^{18}$, I.~Di Sarcina$^{41}$, E.~Diociaiuti$^{40}$, T.~Dorigo$^{10, 61}$, K.~Dreimanis$^{62}$, T.~du Pree$^{63, 64}$, T.~Edgecock$^{25}$, S.~Fabbri$^{1}$, M.~Fabbrichesi$^{43}$, S.~Farinon$^{28}$, G.~Ferrand$^{23}$, J.~A.~Ferreira Somoza$^{1}$, M.~Fieg$^{65}$, F.~Filthaut$^{66, 63}$, P.~Fox$^{13}$, R.~Franceschini$^{67, 68}$, R.~Franqueira Ximenes$^{1}$, M.~Gallinaro$^{56}$, M.~Garcia-Sciveres$^{3}$, L.~Garcia-Tabares$^{69}$, R.~Gargiulo$^{42}$, C.~Garion$^{1}$, M.~V.~Garzelli$^{70}$, M.~Gast$^{71}$, C.~E.~Gerber$^{72}$, L.~Giambastiani$^{35, 10}$, A.~Gianelle$^{10}$, E.~Gianfelice-Wendt$^{13}$, S.~Gibson$^{7}$,S.~Gilardoni$^{1}$, D.~A.~Giove$^{22}$, V.~Giovinco$^{1}$,C.~Giraldin$^{35, 10}$,
A.~Glioti$^{23}$, A.~Gorzawski$^{73, 1}$, M.~Greco$^{68}$, C.~Grojean$^{74}$, A.~Grudiev$^{1}$, E.~Gschwendtner$^{1}$, E.~Gueli$^{11, 11}$, N.~Guilhaudin$^{1}$, C.~Han$^{75}$, T.~Han$^{76}$, J.~M.~Hauptman$^{20}$, M.~Herndon$^{30}$, A.~D.~Hillier$^{29}$, M.~Hillman$^{77}$, T.~R.~Holmes$^{77}$, S.~Homiller$^{78}$, S.~Jana$^{79}$, S.~Jindariani$^{13}$, S.~Johannesson$^{73}$, B.~Johnson$^{77}$, O.~R.~Jones$^{1}$, P.-B.~Jurj$^{80}$, Y.~Kahn$^{13}$, R.~Kamath$^{80}$, A.~Kario$^{64}$, I.~Karpov$^{1}$, D.~Kelliher$^{29}$, W.~Kilian$^{81}$, R.~Kitano$^{82}$, F.~Kling$^{74}$, A.~Kolehmainen$^{1}$, K.~C.~Kong$^{83}$, J.~Kosse$^{16}$, G.~Krintiras$^{83}$, K.~Krizka$^{84}$, N.~Kumar$^{85}$, E.~Kvikne$^{1}$, R.~Kyle$^{86}$, E.~Laface$^{73}$, K.~Lane$^{87}$, A.~Latina$^{1}$, A.~Lechner$^{1}$, J.~Lee$^{19}$, L.~Lee$^{77}$, S.~W.~Lee$^{19}$, T.~Lefevre$^{1}$, E.~Leonardi$^{11}$, G.~Lerner$^{1}$, P.~Li$^{88}$, Q.~Li$^{89}$, T.~Li$^{90}$, W.~Li$^{91}$, R.~Li Voti$^{42, 40}$, M.~Lindroos$^{73}$, R.~Lipton$^{13}$, D.~Liu$^{76}$, M.~Liu$^{1}$, Z.~Liu$^{88}$, A.~Lombardi$^{1}$, S.~Lomte$^{30}$, K.~Long$^{80, 29}$, L.~Longo$^{44}$, J.~Lorenzo$^{92}$, R.~Losito$^{1}$, I.~Low$^{93, 94}$, X.~Lu$^{17}$, D.~Lucchesi$^{35, 10}$, T.~Luo$^{3}$, A.~Lupato$^{35, 10}$, E.~M\'etral$^{1}$, K.~M\k{e}ka{\l}a$^{95, 74}$, Y.~Ma$^{6}$, J.~M.~Ma\'{n}czak$^{1}$, S.~Machida$^{29}$, T.~Madlener$^{74}$, L.~Magaletti$^{96, 44}$, M.~Maggi$^{44}$, H.~Mainaud Durand$^{1}$, F.~Maltoni$^{97, 26, 6}$, M.~Mandurrino$^{9}$, C.~Marchand$^{23}$, F.~Mariani$^{22, 42}$, S.~Marin$^{1}$, S.~Mariotto$^{21, 22}$, S.~Martin-Haugh$^{29}$, M.~R.~Masullo$^{98}$, G.~S.~Mauro$^{46}$, A.~Mazzolari$^{24, 99}$, B.~Mele$^{11}$, F.~Meloni$^{74}$, X.~Meng$^{100}$, M.~Mentink$^{1}$, R.~Miceli$^{26}$, N.~Milas$^{73}$, A.~Mohammadi$^{30}$, D.~Moll$^{55}$, A.~Montella$^{101}$, M.~Morandin$^{10}$, M.~Morrone$^{1}$, T.~Mulder$^{1}$, R.~Musenich$^{28}$, M.~Nardecchia$^{42, 43}$, F.~Nardi$^{35}$, D.~Neuffer$^{13}$, D.~Newbold$^{29}$, D.~Novelli$^{28, 42}$, M.~Olveg\r{a}rd$^{102}$, Y.~Onel$^{103}$, D.~Orestano$^{67, 68}$, J.~Osborne$^{1}$, S.~Otten$^{64}$, Y.~M.~Oviedo Torres$^{104}$, D.~Paesani$^{40, 1}$, S.~Pagan Griso$^{3}$, D.~Pagani$^{6}$, K.~Pal$^{1}$, M.~Palmer$^{27}$, A.~Pampaloni$^{28}$, P.~Panci$^{39, 105}$, P.~Pani$^{74}$, Y.~Papaphilippou$^{1}$, R.~Paparella$^{22}$, P.~Paradisi$^{35, 10}$, A.~Passeri$^{68}$, N.~Pastrone$^{9}$, A.~Pellecchia$^{44}$, F.~Piccinini$^{4}$, H.~Piekarz$^{13}$, T.~Pieloni$^{106}$, J.~Plouin$^{23}$, A.~Portone$^{92}$, K.~Potamianos$^{17}$, J.~Potdevin$^{106, 1}$, S.~Prestemon$^{3}$, T.~Puig$^{107}$, J.~Qiang$^{3}$, L.~Quettier$^{23}$, T.~R.~Rabemananjara$^{108, 63}$, E.~Radicioni$^{44}$, R.~Radogna$^{51, 44}$, I.~C.~Rago$^{11}$, A.~Ratkus$^{62}$, E.~Resseguie$^{3}$, J.~Reuter$^{74}$, P.~L.~Ribani$^{26}$, C.~Riccardi$^{34, 4}$, S.~Ricciardi$^{29}$, T.~Robens$^{109}$, Y.~Robert$^{1}$, C.~Rogers$^{29}$, J.~Rojo$^{63, 108}$, M.~Romagnoni$^{99, 24}$, K.~Ronald$^{86, 38}$, B.~Rosser$^{18}$, C.~Rossi$^{1}$, L.~Rossi$^{21, 22}$, L.~Rozanov$^{18}$, M.~Ruhdorfer$^{110}$, R.~Ruiz$^{111}$, F.~S. Queiroz$^{104, 111}$, S.~Saini$^{47, 1}$, F.~Sala$^{26, 6}$, C.~Salierno$^{26}$, T.~Salmi$^{112}$, P.~Salvini$^{4, 34}$, E.~Salvioni$^{47}$, N.~Sammut$^{113}$, C.~Santini$^{22}$, A.~Saputi$^{24}$, I.~Sarra$^{40}$, G.~Scarantino$^{22, 42}$, H.~Schneider-Muntau$^{114}$, D.~Schulte$^{1}$, J.~Scifo$^{41}$, T.~Sen$^{13}$, C.~Senatore$^{115}$, A.~Senol$^{59}$, D.~Sertore$^{22}$, L.~Sestini$^{10}$, R.~C.~Silva R\^ego$^{104, 111}$, F.~M.~Simone$^{96, 44}$, K.~Skoufaris$^{1}$, G.~Sorbello$^{116, 46}$, M.~Sorbi$^{21, 22}$, S.~Sorti$^{21, 22}$, L.~Soubirou$^{23}$, D.~Spataro$^{74}$, A.~Stamerra$^{51, 44}$, S.~Stapnes$^{1}$, G.~Stark$^{117}$, M.~Statera$^{22}$, B.~M.~Stechauner$^{118, 1}$, S.~Su$^{119}$, W.~Su$^{75}$, X.~Sun$^{89}$, A.~Sytov$^{24}$, J.~Tang$^{75}$, J.~Tang$^{120, 100}$, R.~Taylor$^{1}$, H.~Ten Kate$^{64, 1}$, P.~Testoni$^{92}$, L.~S.~Thiele$^{2, 1}$, R.~Tomas Garcia$^{1}$, M.~Topp-Mugglestone$^{1, 36}$, T.~Torims$^{62, 1}$, R.~Torre$^{28}$, L.~T.~Tortora$^{68, 67}$,
%L.~Tortora$^{68}$,
S.~Trifinopoulos$^{49}$, S.-A.~Udongwo$^{2, 1}$, I.~Vai$^{34, 4}$, R.~U.~Valente$^{22}$, U.~van Rienen$^{2}$, R.~van Weelderen$^{1}$, M.~Vanwelde$^{1}$, G.~Velev$^{13}$, R.~Venditti$^{51, 44}$, A.~Vendrasco$^{77}$, A.~Verna$^{41}$, A.~Verweij$^{1}$, P.~Verwilligen$^{44}$, Y.~Villamzar$^{104}$, L.~Vittorio$^{121}$, P.~Vitulo$^{34, 4}$, I.~Vojskovic$^{73}$, D.~Wang$^{89}$, L.-T.~Wang$^{18}$, X.~Wang$^{122}$, M.~Wendt$^{1}$, M.~Widorski$^{1}$, M.~Wozniak$^{1}$, Y.~Wu$^{123}$, A.~Wulzer$^{124, 125}$, K.~Xie$^{76}$, Y.~Yang$^{126}$, Y.~C.~Yap$^{74}$, K.~Yonehara$^{13}$, H.~D.~Yoo$^{127}$, Z.~You$^{75}$, M.~Zanetti$^{35}$, A.~Zaza$^{51, 44}$, L.~Zhang$^{86}$, R.~Zhu$^{128, 129}$, A.~Zlobin$^{13}$, D.~Zuliani$^{35, 10}$, J.~F.~Zurita$^{130}$

\vspace{3mm}

\begin{flushleft}

{\em\footnotesize
$^{1}$ {\href{https://ror.org/01ggx4157}{European Organization for Nuclear Research}, Geneva, Switzerland}, \\ 
$^{2}$ {\href{https://ror.org/03zdwsf69}{University of Rostock}, Rostock, Germany}, \\ 
$^{3}$ {\href{https://ror.org/02jbv0t02}{Lawrence Berkeley National Laboratory}, Berkeley, CA, United States}, \\ 
$^{4}$ {\href{https://ror.org/01st30669}{INFN Sezione di Pavia}, Pavia, Italy}, \\ 
$^{5}$ {\href{https://ror.org/01wntqw50}{Ankara University}, Ankara, T\"urkiye}, \\ 
$^{6}$ {\href{https://ror.org/04j0x0h93}{INFN Sezione di Bologna}, Bologna, Italy}, \\ 
$^{7}$ {\href{https://ror.org/04g2vpn86}{Royal Holloway University of London}, Egham, United Kingdom}, \\ 
$^{8}$ {\href{https://ror.org/048tbm396}{University of Turin}, Turin, Italy}, \\ 
$^{9}$ {\href{https://ror.org/01vj6ck58}{INFN Sezione di Torino}, Turin, Italy}, \\ 
$^{10}$ {\href{https://ror.org/00z34yn88}{INFN Sezione di Padova}, Padua, Italy}, \\ 
$^{11}$ {\href{https://ror.org/05eva6s33}{INFN Sezione di Roma I}, Rome, Italy}, \\ 
$^{12}$ {\href{https://ror.org/027m9bs27}{University of Manchester}, Manchester, United Kingdom}, \\ 
$^{13}$ {\href{https://ror.org/020hgte69}{Fermi National Accelerator Laboratory}, Batavia, IL, United States}, \\ 
$^{14}$ {\href{https://ror.org/0293rh119}{University of Oregon}, Eugene, OR, United States}, \\ 
$^{15}$ {\href{https://ror.org/023gzwx10}{Fayoum University}, Al Fayy\=um,, Egypt}, \\ 
$^{16}$ {\href{https://ror.org/03eh3y714}{Paul Scherrer Institute}, Villigen, Switzerland}, \\ 
$^{17}$ {\href{https://ror.org/01a77tt86}{University of Warwick}, Coventry, United Kingdom}, \\ 
$^{18}$ {\href{https://ror.org/024mw5h28}{University of Chicago}, Chicago IL, United States America}, \\ 
$^{19}$ {\href{https://ror.org/040c17130}{Kyungpook National University}, Daegu, South Korea}, \\ 
$^{20}$ {\href{https://ror.org/04rswrd78}{Iowa State University}, Ames, IA, United States}, \\ 
$^{21}$ {\href{https://ror.org/00wjc7c48}{University of Milan}, Milan, Italy}, \\ 
%    Universit{"a} degli Studi di Milano, Dipartimento di Fisica, 20133 Milano, Italy, \\ 
$^{22}$ {\href{https://ror.org/05s4gph86}{Laboratorio LASA}, Segrate, Italy}, \\ 
%    Laboratory for Accelerator and Applied Superconductivity, INFN, V. F.lli Cervi 201, 20054 Segrate, Italy, \\ 
$^{23}$ {\href{https://ror.org/05k705z76}{Institut de recherche sur les lois fondamentales de l'Univers}, Gif-sur-Yvette, France}, \\ 
%    IRFU, CEA, Universit\'e Paris-Saclay}, France, \\ 
$^{24}$ {\href{https://ror.org/00zs3y046}{INFN Sezione di Ferrara}, Ferrara ,Italy}, \\ 
$^{25}$ {\href{https://ror.org/05t1h8f27}{University of Huddersfield}, Huddersfield, United Kingdom}, \\ 
$^{26}$ {\href{https://ror.org/01111rn36}{University of Bologna}, Bologna, Italy}, \\ 
%    Universit{\'a} degli Studi di Bologna, Via Zamboni, 33, I-40126 Bologna, Italy, \\ 
$^{27}$ {\href{https://ror.org/02ex6cf31}{Brookhaven National Laboratory}, Upton, NY, United States}, \\ 
$^{28}$ {\href{https://ror.org/02v89pq06}{Istituto Nazionale di Fisica Nucleare}, Genova, Italy}, \\ 
$^{29}$ {\href{https://ror.org/01t8fg661}{ISIS Neutron and Muon Source}, Didcot, United Kingdom}, \\ 
$^{30}$ {\href{https://ror.org/01y2jtd41}{University of Wisconsin-Madison}, Madison, WI, United States}, \\ 
$^{31}$ {\href{https://ror.org/02vwzrd76}{Thomas Jefferson National Accelerator Facility}, Newport News, VA,  United States}, \\ 
$^{32}$ \href{https://ror.org/04w4m6z96}{INFN Sezione di Milano}, Milan,Italy, \\ 
$^{33}$ \href{https://ror.org/04mhzgx49}{Tel Aviv University}, Tel Aviv, Israel, \\ 
%    School of Physics and Astronomy, Tel-Aviv University, Tel-Aviv 69978, Israel, \\ 
$^{34}$ \href{https://ror.org/00s6t1f81}{University of Pavia}, Pavia, Italy, \\ 
%    Universit\'a degli Studi di Pavia, Dipartimento di Fisica via Bassi 6, 27100, Pavia, Italy, \\ 
$^{35}$ \href{https://ror.org/00240q980}{University of Padua}, Padua, Italy, \\ 
%    Universit{"a} degli Studi di Padova, via Marzolo\ 8, 35100 Padova, Italy, \\ 
$^{36}$ \href{https://ror.org/00wgpgb78}{John Adams Institute for Accelerator Science}, Oxford, United Kingdom, \\ 
$^{37}$ \href{https://ror.org/04f2nsd36}{Lancaster University}, Lancaster, United Kingdom, \\
% from here until 109, one unit added
$^{38}$ \href{https://ror.org/02a5smf05}{Cockcroft Institute}, Daresbury, United Kingdom, \\ 
$^{39}$ \href{https://ror.org/05symbg58}{INFN Sezione di Pisa}, Pisa, Italy, \\ 
$^{40}$ \href{https://ror.org/049jf1a25}{National Laboratory of Frascati}, Frascati, Italy, \\ 
$^{41}$ \href{https://ror.org/02an8es95}{National Agency for New Technologies,  Energy and Sustainable Economic Development}, Rome, Italy, \\ 
$^{42}$ \href{https://ror.org/02be6w209}{Sapienza University of Rome}, Rome,Italy, \\ 
$^{43}$ \href{https://ror.org/05j3snm48}{INFN Sezione di Trieste}, Trieste, Italy, \\ 
$^{44}$ \href{https://ror.org/022hq6c49}{INFN Sezione di Bari}, Bari, Italy, \\ 
$^{45}$ \href{https://ror.org/04pmn0e78}{Universidad de Alcal\'a}, Alcal\'a de Henares, Spain, \\ 
$^{46}$ \href{https://ror.org/02k1zhm92}{Laboratori Nazionali del Sud}, Catania, Italy, \\ 
$^{47}$ \href{https://ror.org/00ayhx656}{University of Sussex}, Brighton, United Kingdom, \\ 
%    $^{47}$ \href{https://ror.org/05symbg58}{INFN Sezione di Pisa}, Pisa, Italy, \\
$^{48}$ \href{https://ror.org/01tevnk56}{University of Siena}, Siena, Italy,\\
$^{49}$ \href{https://ror.org/042nb2s44}{Massachusetts Institute of Technology}, Cambridge, MA,  United States, \\
$^{50}$ \href{https://ror.org/00bgk9508}{Polytechnic University of Turin}, Turin, Italy, \\ %{NEMO Group, Dipartimento Energia, Politecnico di Torino.\ Corso Duca degli Abruzzi, 24, 10129 Torino, Italy}, \\
$^{51}$ \href{https://ror.org/027ynra39}{University of Bari Aldo Moro}, Bari, Italy, \\
%    {Universit\'a  di Bari, Dipartimento di Fisica, Via Amendola 173, I-70125 Bari, Italy}, \\
$^{52}$ \href{https://ror.org/013m0ej23}{Perimeter Institute}, Waterloo, ON, Canada, \\
$^{53}$ \href{https://ror.org/02t274463}{University of California, Santa Barbara}, Santa Barbara, CA, United States, \\
$^{54}$ \href{https://ror.org/03dbr7087}{University of Toronto}, Toronto, ON, Canada, \\
$^{55}$ \href{https://ror.org/05n911h24}{Technical University of Darmstadt}, Darmstadt, Germany, \\ 
%    {Institute for Accelerator Science and Electromagnetic Fields, Technische Universit{"a}t Darmstadt, Schlossgartenstr. 8, 64289 Darmstadt, Germany}, \\
$^{56}$ \href{https://ror.org/01hys1667}{LIP---Laboratory of Instrumentation and Experimental Particle Physics}, Lisbon, Portugal, \\
%    {LIP, Laborat\'{o}rio de Instrumenta\c{c}\~{a}o e F\'{i}sica Experimental de Part\'{i}culas, Lisbon, Portugal}, \\
$^{57}$ \href{https://ror.org/04njjy449}{Universidad de Granada}, Granada, Spain, \\  
$^{58}$ \href{https://ror.org/02vv5y108}{INFN Sezione di Firenze}, Sesto Fiorentino, Italy, \\
$^{59}$ \href{https://ror.org/01x1kqx83}{Bolu Abant Izzet Baysal University}, Bolu, T\"{u}rkiye, \\
$^{60}$ \href{https://ror.org/01kg8sb98}{Indiana University}, Bloomington, IN, United States, \\
$^{61}$ \href{https://ror.org/016st3p78}{Lule\.a University of Technology}, Lule\.a, Sweden, \\ 
$^{62}$ \href{https://ror.org/00twb6c09}{Riga Technical University}, Riga, Latvia, \\
$^{63}$ \href{https://ror.org/00f9tz983}{National Institute for Subatomic Physics}, Amsterdam, Netherlands, \\
$^{64}$ \href{https://ror.org/006hf6230}{University of Twente}, Enschede, Netherlands, \\  
$^{65}$ \href{https://ror.org/04gyf1771}{University of California, Irvine}, Irvine, CA, United States, \\
$^{66}$ \href{https://ror.org/016xsfp80}{Radboud University Nijmegen}, Nijmegen, Netherlands, \\
$^{67}$ \href{https://ror.org/05vf0dg29}{Roma Tre University}, Rome, Italy, \\ %{Universit\`a degli Studi di Roma Tre, Dipartimento di Matematica e Fisica, Via Vasca Navale 84, I-00146 Roma, Rome, Italy}
$^{68}$ \href{https://ror.org/009wnjh50}{INFN Sezione di Roma III}, Rome, Italy, \\ 
$^{69}$ \href{https://ror.org/05xx77y52}{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnologicas}, Madrid, Spain, \\ 
$^{70}$ \href{https://ror.org/00g30e956}{Universit\"at Hamburg}, Hamburg, Germany, \\
$^{71}$ \href{https://ror.org/04t3en479}{Karlsruhe Institute of Technology}, Karlsruhe, Germany, \\ %Karlsruher Institut f{"u}r Technologie (KIT), Kaiserstraße 12, 76131 Karlsruhe, Germany, \\
$^{72}$ \href{https://ror.org/02mpq6x41}{University of Illinois at Chicago}, Chicago, IL,  United States, \\
$^{73}$ \href{https://ror.org/01wv9cn34}{European Spallation Source}, Lund, Sweden, \\
$^{74}$ \href{https://ror.org/01js2sh04}{Deutsches Elektronen-Synchrotron DESY}, Hamburg, Germany, \\
$^{75}$ \href{https://ror.org/0064kty71}{Sun Yat-sen University}, Guangzhou, China, \\ 
$^{76}$ \href{https://ror.org/01an3r305}{University of Pittsburgh}, Pittsburgh, PA, United States, \\
$^{77}$ \href{https://ror.org/020f3ap87}{University of Tennessee at Knoxville}, Knoxville, TN, United States, \\ 
$^{78}$ \href{https://ror.org/03vek6s52}{Harvard University}, Cambridge, MA, United States, \\ 
$^{79}$ \href{https://ror.org/052d0h423}{Max Planck Institute for Nuclear Physics}, Heidelberg, Germany, \\ %Max-Planck-Institut f{\"u}r Kernphysik,  Saupfercheckweg 1, 69117 Heidelberg, Germany, \\
$^{80}$ \href{https://ror.org/041kmwe10}{Imperial College London}, London, United Kingdom, \\
$^{81}$ \href{https://ror.org/02azyry73}{University of Siegen}, Siegen, Germany, \\ 
$^{82}$ \href{https://ror.org/01g5y5k24}{High Energy Accelerator Research Organization}, Tsukuba, Japan, \\ 
$^{83}$ \href{https://ror.org/001tmjg57}{University of Kansas}, Lawrence, KS, United States, \\
$^{84}$ \href{https://ror.org/03angcq70}{University of Birmingham}, Birmingham, United Kingdom, \\
$^{85}$ \href{https://ror.org/04kf25f32}{Shree Guru Gobind Singh Shree Guru Gobind Singh Tricentenary University}, Gurgaon, India, \\
$^{86}$ \href{https://ror.org/00n3w3b69}{University of Strathclyde}, Glasgow, United Kingdom, \\
$^{87}$ \href{https://ror.org/05qwgg493}{Boston University}, Boston, MA, United States, \\
$^{88}$ \href{https://ror.org/017zqws13}{University of Minnesota}, Minneapolis, MN,  United States, \\
$^{89}$ \href{https://ror.org/02v51f717}{Peking University}, Beijing, China, \\ 
$^{90}$ \href{https://ror.org/01y1kjr75}{Nankai University}, Tianjin, China, \\ 
$^{91}$ \href{https://ror.org/008zs3103}{Rice University}, Houston, TX, United States, \\ 
$^{92}$ \href{https://ror.org/02q40pc92}{Fusion for Energy}, Barcelona, Spain, \\ 
$^{93}$ \href{https://ror.org/000e0be47}{Northwestern University}, Evanston, IL, United States, \\ 
$^{94}$ \href{https://ror.org/05gvnxz63}{Argonne National Laboratory}, Lemont, IL, United States, \\ 
$^{95}$ \href{https://ror.org/039bjqg32}{University of Warsaw}, Warsaw, Poland, \\ 
$^{96}$ \href{https://ror.org/03c44v465}{Polytechnic University of Bari}, Bari, Italy, \\ 
$^{97}$ \href{https://ror.org/02495e989}{UCLouvain}, Louvain-la-Neuve, Belgium, \\ 
%    {Center for Cosmology, Particle Physics and Phenomenology, Université Catholique de Louvain, Louvain-la-Neuve, Belgium}, \\ 
$^{98}$ \href{https://ror.org/015kcdd40}{INFN  Sezione di Napoli}, Naples, Italy, \\ 
$^{99}$ \href{https://ror.org/041zkgm14}{University of Ferrara}, Ferrara, Italy, \\ 
$^{100}$ \href{https://ror.org/03v8tnc06}{Institute of High Energy Physics}, Beijing, China, \\ 
$^{101}$ \href{https://ror.org/05f0yaq80}{Stockholm University},Stockholm, Sweden, \\ 
%   $^{101}$ \href{https://ror.org/039bjqg32}{University of Warsaw}, Warsaw, Poland, \\ 
$^{102}$ \href{https://ror.org/048a87296}{Uppsala University}, Uppsala, Sweden, \\ 
$^{103}$ \href{https://ror.org/036jqmy94}{University of Iowa}, Iowa City, IA, United States, \\ 
$^{104}$ \href{https://ror.org/04wn09761}{Universidade Federal do Rio Grande do Norte, Campus Universit\'ario}, Natal, Brazil, \\ 
$^{105}$ \href{https://ror.org/03ad39j10}{University of Pisa}, Pisa, Italy, \\ 
$^{106}$ \href{https://ror.org/02s376052}{\'Ecole polytechnique f\'ed\'erale de Lausanne}, Lausanne, Switzerland, \\ 
$^{107}$ \href{https://ror.org/03hasqf61}{Institut de Ciencia de Materials de Barcelona}, Cerdanyola del Vall\`es, Spain, \\ 
$^{108}$ \href{https://ror.org/008xxew50}{Vrije Universiteit Amsterdam}, Amsterdam, Netherlands, \\ 
$^{109}$ \href{https://ror.org/02mw21745}{Rudjer Boskovic Institute}, Zagreb, Croatia, \\ 
%    $^{109}$ \href{https://ror.org/02a5smf05}{Cockcroft Institute}, Daresbury, United Kingdom, \\ 
$^{110}$ \href{https://ror.org/05bnh6r87}{Cornell University}, Ithaca, NY, United States, \\ 
$^{111}$ \href{https://ror.org/01n78t774}{Institute of Nuclear Physics, Polish Academy of Sciences}, Krak{\'o}w, Poland, \\ 
%    $^{112}$ \href{https://ror.org/04wn09761}{Universidade Federal do Rio Grande do Norte, Campus Universit\'ario}, Natal, Brazil, \\ 
$^{112}$ \href{https://ror.org/033003e23}{Tampere University}, Tampere, Finland, \\ 
$^{113}$ \href{https://ror.org/03a62bv60}{University of Malta}, Msida, Malta, \\ 
$^{114}$ {CS\&T, France}, \\ 
$^{115}$ \href{https://ror.org/01swzsf04}{University of Geneva}, Geneva, Switzerland, \\ 
$^{116}$ \href{https://ror.org/03a64bh57}{University of Catania}, Catania, Italy, \\ 
$^{117}$ \href{https://ror.org/03s65by71}{University of California, Santa Cruz}, Santa Cruz, CA, United States, \\ 
$^{118}$ \href{https://ror.org/04d836q62}{TU Wien}, Vienna, Austria, \\ 
$^{119}$ \href{https://ror.org/03m2x1q45}{University of Arizona}, Tucson, AZ, United States, \\ 
$^{120}$ \href{https://ror.org/04c4dkn09}{University of Science and Technology of China}, Hefei, China, \\
$^{121}$ \href{https://lapp.in2p3.fr}{Laboratoire d’Annecy de Physique des Particules LAPP}, Annecy, France, \\
%    $^{121}$ {LAPTh, Universit\'{e} Savoie Mont-Blanc et CNRS, Annecy, France}, \\ 
$^{122}$ \href{https://ror.org/0168r3w48}{University of California, San Diego}, La Jolla, CA, United States, \\ 
$^{123}$ \href{https://ror.org/036trcv74}{Nanjing Normal University}, Nanjing, China, \\ 
$^{124}$ \href{https://ror.org/0371hy230}{Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats}, Barcelona, Spain, \\ 
$^{125}$ \href{https://ror.org/03kpps236}{Barcelona Institute for Science and Technology}, Barcelona, Spain, \\
$^{126}$ \href{https://ror.org/01ryk1543}{University of Southampton}, Southampton, United Kingdom, \\ 
$^{127}$ \href{https://ror.org/01wjejq96}{Yonsei University}, Seoul, South Korea, \\ 
$^{128}$ \href{https://ror.org/03x8rhq63}{Institute of Modern Physics}, Lanzhou, China, \\ 
$^{129}$ \href{https://ror.org/05qbk4x57}{University of Chinese Academy of Sciences}, Beijing, China, \\ 
$^{130}$ \href{https://ror.org/017xch102}{Instituto de F\'{\i}sica Corpuscular}, Paterna, Spain
%    CSIC-Universitat de Val\`encia,   Catedr\'{a}tico Jos\'{e} Beltr\'{a}n 2, E-46980, Paterna, Spain
}
\end{flushleft}

%\newpage

%\thispagestyle{empty}
%\mbox{}
%\vfill



==> AddAuthors/AddAuthors_old2.tex <==
\newpage 
\thispagestyle{empty}

\vskip 10cm
\begin{center}
{\huge\bfseries
Interim report for the \\
International Muon Collider Collaboration (IMCC) }

\end{center}

\vspace{5mm}
{\small\ref{}
\noindent
C.~Accettura$^{1}$, S.~Adrian$^{2}$, R.~Agarwal$^{3}$, C.~Ahdida$^{1}$, C.~Aim\'e$^{4}$, A.~Aksoy$^{1, 5}$, G.~L.~Alberghi$^{6}$, S.~Alden$^{7}$, N.~Amapane$^{8, 9}$, D.~Amorim$^{1}$, P.~Andreetto$^{10}$, F.~Anulli$^{11}$, R.~Appleby$^{12}$, A.~Apresyan$^{13}$, P.~Asadi$^{14}$, M.~Attia Mahmoud$^{15}$, B.~Auchmann$^{16, 1}$, J.~Back$^{17}$, A.~Badea$^{18}$, K.~J.~Bae$^{19}$, E.~J.~Bahng$^{20}$, L.~Balconi$^{21, 22}$, F.~Balli$^{23}$, L.~Bandiera$^{24}$, C.~Barbagallo$^{1}$, R.~Barlow$^{25}$, C.~Bartoli$^{26}$, N.~Bartosik$^{9}$, E.~Barzi$^{13}$, F.~Batsch$^{1}$, M.~Bauce$^{11}$, M.~Begel$^{27}$, J.~S.~Berg$^{27}$, A.~Bersani$^{28}$, A.~Bertarelli$^{1}$, F.~Bertinelli$^{1}$, A.~Bertolin$^{10}$, P.~Bhat$^{13}$, C.~Bianchi$^{26}$, M.~Bianco$^{1}$, W.~Bishop$^{17, 29}$, K.~Black$^{30}$, F.~Boattini$^{1}$, A.~Bogacz$^{31}$, M.~Bonesini$^{32}$, B.~Bordini$^{1}$, P.~Borges de Sousa$^{1}$, S.~Bottaro$^{33}$, L.~Bottura$^{1}$, S.~Boyd$^{17}$, M.~Breschi$^{26, 6}$, F.~Broggi$^{22}$, M.~Brunoldi$^{34, 4}$, X.~Buffat$^{1}$, L.~Buonincontri$^{35, 10}$, P.~N.~Burrows$^{36}$, G.~C.~Burt$^{37}$, D.~Buttazzo$^{38}$, B.~Caiffi$^{28}$, S.~Calatroni$^{1}$, M.~Calviani$^{1}$, S.~Calzaferri$^{34}$, D.~Calzolari$^{1}$, C.~Cantone$^{39}$, R.~Capdevilla$^{13}$, C.~Carli$^{1}$, C.~Carrelli$^{40}$, F.~Casaburo$^{41, 11}$, M.~Casarsa$^{42}$, L.~Castelli$^{41, 11}$, M.~G.~Catanesi$^{43}$, L.~Cavallucci$^{26, 6}$, G.~Cavoto$^{41, 11}$, F.~G.~Celiberto$^{44}$, L.~Celona$^{45}$, A.~Cemmi$^{40}$, S.~Ceravolo$^{39}$, A.~Cerri$^{46, 47, 38}$, F.~Cerutti$^{1}$, G.~Cesarini$^{39}$, C.~Cesarotti$^{48}$, A.~Chanc\'e$^{23}$, N.~Charitonidis$^{1}$, M.~Chiesa$^{4}$, P.~Chiggiato$^{1}$, V.~L.~Ciccarella$^{39, 41}$, P.~Cioli~Puviani$^{49}$, A.~Colaleo$^{50, 43}$, F.~Colao$^{40}$, F.~Collamati$^{11}$, M.~Costa$^{51}$, N.~Craig$^{52}$, D.~Curtin$^{53}$, L.~D'Angelo$^{54}$, G.~Da~Molin$^{55}$, H.~Damerau$^{1}$, S.~Dasu$^{30}$, J.~de Blas$^{56}$, S.~De Curtis$^{57}$, H.~De~Gersem$^{54}$, T.~Del Moro$^{41, 40}$, J.-P.~Delahaye$^{1}$, D.~Denisov$^{27}$, H.~Denizli$^{58}$, R.~Dermisek$^{59}$, P.~Desir\'e~Valdor$^{1}$, C.~Desponds$^{1}$, L.~Di~Luzio$^{10}$, E.~Di~Meco$^{39}$, K.~F.~Di~Petrillo$^{18}$, I.~Di~Sarcina$^{40}$, E.~Diociaiuti$^{39}$, T.~Dorigo$^{10, 60}$, K.~Dreimanis$^{61}$, T.~du~Pree$^{62, 63}$, T.~Edgecock$^{25}$, S.~Fabbri$^{1}$, M.~Fabbrichesi$^{42}$, S.~Farinon$^{28}$, G.~Ferrand$^{23}$, J.~A.~Ferreira~Somoza$^{1}$, M.~Fieg$^{64}$, F.~Filthaut$^{65, 62}$, P.~Fox$^{13}$, R.~Franceschini$^{66, 67}$, R.~Franqueira~Ximenes$^{1}$, M.~Gallinaro$^{55}$, M.~Garcia-Sciveres$^{3}$, L.~Garcia-Tabares$^{68}$, R.~Gargiulo$^{41}$, C.~Garion$^{1}$, M.~V.~Garzelli$^{69}$, M.~Gast$^{70}$, C.~E.~Gerber$^{71}$, L.~Giambastiani$^{35, 10}$, A.~Gianelle$^{10}$, E.~Gianfelice-Wendt$^{13}$, S.~Gibson$^{7}$, S.~Gilardoni$^{1}$, D.~A.~Giove$^{22}$, V.~Giovinco$^{1}$, A.~Glioti$^{23}$, A.~Gorzawski$^{72, 1}$, M.~Greco$^{67}$, C.~Grojean$^{73}$, A.~Grudiev$^{1}$, E.~Gschwendtner$^{1}$, E.~Gueli$^{11}$, N.~Guilhaudin$^{1}$, C.~Han$^{74}$, T.~Han$^{75}$, J.~M.~Hauptman$^{20}$, M.~Herndon$^{30}$, A.~D.~Hillier$^{29}$, M.~Hillman$^{76}$, T.~R.~Holmes$^{76}$, S.~Homiller$^{77}$, S.~Jana$^{78}$, S.~Jindariani$^{13}$, S.~Johannesson$^{72}$, B.~Johnson$^{76}$, O.~R.~Jones$^{1}$, P.-B.~Jurj$^{79}$, Y.~Kahn$^{13}$, R.~Kamath$^{79}$, A.~Kario$^{63}$, I.~Karpov$^{1}$, D.~Kelliher$^{29}$, W.~Kilian$^{80}$, R.~Kitano$^{81}$, F.~Kling$^{73}$, A.~Kolehmainen$^{1}$, K.~Kong$^{82}$, J.~Kosse$^{16}$, G.~Krintiras$^{82}$, K.~Krizka$^{83}$, N.~Kumar$^{84}$, E.~Kvikne$^{1}$, R.~Kyle$^{85}$, E.~Laface$^{72}$, K.~Lane$^{86}$, A.~Latina$^{1}$, A.~Lechner$^{1}$, J.~Lee$^{19}$, L.~Lee$^{76}$, S.~W.~Lee$^{19}$, T.~Lefevre$^{1}$, E.~Leonardi$^{11}$, G.~Lerner$^{1}$, P.~Li$^{87}$, Q.~Li$^{88}$, T.~Li$^{89}$, W.~Li$^{90}$, R.~Li~Voti$^{41, 39}$, M.~Lindroos$^{72}$, R.~Lipton$^{13}$, D.~Liu$^{75}$, M.~Liu$^{1}$, Z.~Liu$^{91}$, A.~Lombardi$^{1}$, S.~Lomte$^{30}$, K.~Long$^{79, 29}$, L.~Longo$^{43}$, J.~Lorenzo$^{92}$, R.~Losito$^{1}$, I.~Low$^{93, 94}$, X.~Lu$^{17}$, D.~Lucchesi$^{35, 10}$, T.~Luo$^{3}$, A.~Lupato$^{35, 10}$, Y.~Ma$^{6}$, S.~Machida$^{29}$, T.~Madlener$^{73}$, L.~Magaletti$^{95, 43, 95}$, M.~Maggi$^{43}$, H.~Mainaud~Durand$^{1}$, F.~Maltoni$^{96, 26, 6}$, J.~M.~Manczak$^{1}$, M.~Mandurrino$^{9}$, C.~Marchand$^{23}$, F.~Mariani$^{22, 41}$, S.~Marin$^{1}$, S.~Mariotto$^{21, 22}$, S.~Martin-Haugh$^{29}$, M.~R.~Masullo$^{97}$, G.~S.~Mauro$^{45}$, A.~Mazzolari$^{24, 98}$, B.~Mele$^{11}$, F.~Meloni$^{73}$, X.~Meng$^{99}$, M.~Mentink$^{1}$, E.~M\'etral$^{1}$, R.~Miceli$^{26}$, N.~Milas$^{72}$, A.~Mohammadi$^{30}$, D.~Moll$^{54}$, A.~Montella$^{100}$, M.~Morandin$^{10}$, M.~Morrone$^{1}$, T.~Mulder$^{1}$, R.~Musenich$^{28}$, K.~M\k{e}ka{\l}a$^{101, 73}$, M.~Nardecchia$^{41, 42}$, F.~Nardi$^{35}$, D.~Neuffer$^{13}$, D.~Newbold$^{29}$, D.~Novelli$^{28, 41}$, M.~Olveg\r{a}rd$^{102}$, Y.~Onel$^{103}$, D.~Orestano$^{66, 67}$, J.~Osborne$^{1}$, S.~Otten$^{63}$, Y.~M.~Oviedo~Torres$^{104}$, D.~Paesani$^{39, 1}$, S.~Pagan~Griso$^{3}$, D.~Pagani$^{6}$, K.~Pal$^{1}$, M.~Palmer$^{27}$, A.~Pampaloni$^{28}$, P.~Panci$^{38, 105}$, P.~Pani$^{73}$, Y.~Papaphilippou$^{1}$, R.~Paparella$^{22}$, P.~Paradisi$^{35, 10}$, A.~Passeri$^{67}$, N.~Pastrone$^{9}$, A.~Pellecchia$^{43}$, F.~Piccinini$^{4}$, H.~Piekarz$^{13}$, T.~Pieloni$^{106}$, J.~Plouin$^{23}$, A.~Portone$^{92}$, K.~Potamianos$^{17}$, J.~Potdevin$^{106, 1}$, S.~Prestemon$^{3}$, T.~Puig$^{107}$, J.~Qiang$^{3}$, L.~Quettier$^{23}$, T.~R.~Rabemananjara$^{108, 62}$, E.~Radicioni$^{43}$, R.~Radogna$^{50, 43}$, I.~C.~Rago$^{11}$, A.~Ratkus$^{61}$, E.~Resseguie$^{3}$, J.~Reuter$^{73}$, P.~L.~Ribani$^{26}$, C.~Riccardi$^{34, 4}$, S.~Ricciardi$^{29}$, T.~Robens$^{109}$, Y.~Robert$^{1}$, C.~Rogers$^{29}$, J.~Rojo$^{62, 108}$, M.~Romagnoni$^{98, 24}$, K.~Ronald$^{85, 110}$, B.~Rosser$^{18}$, C.~Rossi$^{1}$, L.~Rossi$^{21, 22}$, L.~Rozanov$^{18}$, M.~Ruhdorfer$^{111}$, R.~Ruiz$^{112}$, F.~S. Queiroz$^{104, 113}$, S.~Saini$^{46, 1}$, F.~Sala$^{26, 6}$, C.~Salierno$^{26}$, T.~Salmi$^{114}$, P.~Salvini$^{4, 34}$, E.~Salvioni$^{46}$, N.~Sammut$^{115}$, C.~Santini$^{22}$, A.~Saputi$^{24}$, I.~Sarra$^{39}$, G.~Scarantino$^{22, 41}$, H.~Schneider-Muntau$^{116}$, D.~Schulte$^{1}$, J.~Scifo$^{40}$, T.~Sen$^{13}$, C.~Senatore$^{117}$, A.~Senol$^{58}$, D.~Sertore$^{22}$, L.~Sestini$^{10}$, R.~C.~Silva RÃªgo$^{104, 113}$, F.~M.~Simone$^{95, 43}$, K.~Skoufaris$^{1}$, G.~Sorbello$^{118, 45}$, M.~Sorbi$^{21, 22}$, S.~Sorti$^{21, 22}$, L.~Soubirou$^{23}$, D.~Spataro$^{73}$, A.~Stamerra$^{50, 43}$, S.~Stapnes$^{1}$, G.~Stark$^{119}$, M.~Statera$^{22}$, B.~M.~Stechauner$^{120, 1}$, S.~Su$^{121}$, W.~Su$^{74}$, X.~Sun$^{88}$, A.~Sytov$^{24}$, J.~Tang$^{74}$, J.~Tang$^{122, 99}$, R.~Taylor$^{1}$, H.~Ten Kate$^{63, 1}$, P.~Testoni$^{92}$, L.~S.~Thiele$^{2, 1}$, R.~Tomas Garcia$^{1}$, M.~Topp-Mugglestone$^{1, 36}$, T.~Torims$^{61, 1}$, R.~Torre$^{28}$, L.~T.~Tortora$^{67, 66}$, L.~Tortora$^{67}$, S.~Trifinopoulos$^{48}$, S.-A.~Udongwo$^{2, 1}$, I.~Vai$^{34, 4}$, R.~U.~Valente$^{22}$, U.~van Rienen$^{2}$, R.~Van Weelderen$^{1}$, M.~Vanwelde$^{1}$, G.~Velev$^{13}$, R.~Venditti$^{50, 43}$, A.~Vendrasco$^{76}$, A.~Verna$^{40}$, A.~Verweij$^{1}$, P.~Verwilligen$^{43}$, Y.~Villamzar$^{104}$, L.~Vittorio$^{123}$, P.~Vitulo$^{34, 4}$, I.~Vojskovic$^{72}$, D.~Wang$^{88}$, L.-T.~Wang$^{18}$, X.~Wang$^{124}$, M.~Wendt$^{1}$, M.~Widorski$^{1}$, M.~Wozniak$^{1}$, Y.~Wu$^{125}$, A.~Wulzer$^{126, 127}$, K.~Xie$^{75}$, Y.~Yang$^{128}$, Y.~C.~Yap$^{73}$, K.~Yonehara$^{13}$, H.~D.~Yoo$^{129}$, Z.~You$^{74}$, M.~Zanetti$^{35}$, A.~Zaza$^{50, 43}$, L.~Zhang$^{85}$, R.~Zhu$^{130, 131}$, A.~Zlobin$^{13}$, D.~Zuliani$^{35, 10}$, J.~F.~Zurita$^{132}$ }

\vspace{3mm}

\begin{flushleft}

{\em\footnotesize
$^{1}$ {\href{https://ror.org/01ggx4157}{European Organization for Nuclear Research}, Geneva, Switzerland}, \\ 
$^{2}$ {\href{https://ror.org/03zdwsf69}{University of Rostock}, Rostock, Germany}, \\ 
$^{3}$ {\href{https://ror.org/02jbv0t02}{Lawrence Berkeley National Laboratory}, Berkeley, CA, United States}, \\ 
$^{4}$ {\href{https://ror.org/01st30669}{INFN Sezione di Pavia}, Pavia, Italy}, \\ 
$^{5}$ {\href{https://ror.org/01wntqw50}{Ankara University}, Ankara, T\"urkiye}, \\ 
$^{6}$ {\href{https://ror.org/04j0x0h93}{INFN Sezione di Bologna}, Bologna, Italy}, \\ 
$^{7}$ {\href{https://ror.org/04g2vpn86}{Royal Holloway University of London}, Egham, United Kingdom}, \\ 
$^{8}$ {\href{https://ror.org/048tbm396}{University of Turin}, Turin, Italy}, \\ 
$^{9}$ {\href{https://ror.org/01vj6ck58}{INFN Sezione di Torino}, Turin, Italy}, \\ 
$^{10}$ {\href{https://ror.org/00z34yn88}{INFN Sezione di Padova}, Padua, Italy}, \\ 
$^{11}$ {\href{https://ror.org/05eva6s33}{INFN Sezione di Roma I}, Rome, Italy}, \\ 
$^{12}$ {\href{https://ror.org/027m9bs27}{University of Manchester}, Manchester, United Kingdom}, \\ 
$^{13}$ {\href{https://ror.org/020hgte69}{Fermi National Accelerator Laboratory}, Batavia, IL, United States}, \\ 
$^{14}$ {\href{https://ror.org/0293rh119}{University of Oregon}, Eugene, OR, United States}, \\ 
$^{15}$ {\href{https://ror.org/023gzwx10}{Fayoum University}, Al Fayy\=um,, Egypt}, \\ 
$^{16}$ {\href{https://ror.org/03eh3y714}{Paul Scherrer Institute}, Villigen, Switzerland}, \\ 
$^{17}$ {\href{https://ror.org/01a77tt86}{University of Warwick}, Coventry, United Kingdom}, \\ 
$^{18}$ {\href{https://ror.org/024mw5h28}{University of Chicago}, Chicago IL, United States America}, \\ 
$^{19}$ {\href{https://ror.org/040c17130}{Kyungpook National University}, Daegu, South Korea}, \\ 
$^{20}$ {\href{https://ror.org/04rswrd78}{Iowa State University}, Ames, IA, United States}, \\ 
$^{21}$ {\href{https://ror.org/00wjc7c48}{University of Milan}, Milan, Italy}, \\ %Universit{"a} degli Studi di Milano, Dipartimento di Fisica, 20133 Milano, Italy, \\ 
$^{22}$ {\href{https://ror.org/05s4gph86}{Laboratorio LASA}, Segrate, Italy}, \\ %Laboratory for Accelerator and Applied Superconductivity, INFN, V. F.lli Cervi 201, 20054 Segrate, Italy, \\ 
$^{23}$ {\href{https://ror.org/05k705z76}{Institut de recherche sur les lois fondamentales de l'Univers}, Gif-sur-Yvette, France}, \\ %IRFU, CEA, Universit\'e Paris-Saclay}, France, \\ 
$^{24}$ {\href{https://ror.org/00zs3y046}{INFN Sezione di Ferrara}, Ferrara ,Italy}, \\ 
$^{25}$ {\href{https://ror.org/05t1h8f27}{University of Huddersfield}, Huddersfield, United Kingdom}, \\ 
$^{26}$ {\href{https://ror.org/01111rn36}{University of Bologna}, Bologna, Italy}, \\ %Universit{\'a} degli Studi di Bologna, Via Zamboni, 33, I-40126 Bologna, Italy, \\ 
$^{27}$ {\href{https://ror.org/02ex6cf31}{Brookhaven National Laboratory}, Upton, NY, United States}, \\ 
$^{28}$ {\href{https://ror.org/02v89pq06}{Istituto Nazionale di Fisica Nucleare}, Genova, Italy}, \\ 
$^{29}$ {\href{https://ror.org/01t8fg661}{ISIS Neutron and Muon Source}, Didcot, United Kingdom}, \\ 
$^{30}$ {\href{https://ror.org/01y2jtd41}{University of Wisconsin-Madison}, Madison, WI, United States}, \\ 
$^{31}$ {\href{https://ror.org/02vwzrd76}{Thomas Jefferson National Accelerator Facility}, Newport News, VA,  United States}, \\ 
$^{32}$ \href{https://ror.org/04w4m6z96}{INFN Sezione di Milano}, Milan,Italy, \\ 
$^{33}$ \href{https://ror.org/04mhzgx49}{Tel Aviv University}, Tel Aviv, Israel, \\ %School of Physics and Astronomy, Tel-Aviv University, Tel-Aviv 69978, Israel, \\ 
$^{34}$ \href{https://ror.org/00s6t1f81}{University of Pavia}, Pavia, Italy, \\ %Universit\'a degli Studi di Pavia, Dipartimento di Fisica via Bassi 6, 27100, Pavia, Italy, \\ 
$^{35}$ \href{https://ror.org/00240q980}{University of Padua}, Padua, Italy, \\ %Universit{"a} degli Studi di Padova, via Marzolo\ 8, 35100 Padova, Italy, \\ 
$^{36}$ \href{https://ror.org/00wgpgb78}{John Adams Institute for Accelerator Science}, Oxford, United Kingdom, \\ 
$^{37}$ \href{https://ror.org/02a5smf05}{Cockcroft Institute}, Daresbury, United Kingdom, \\ 
$^{38}$ \href{https://ror.org/05symbg58}{INFN Sezione di Pisa}, Pisa, Italy, \\ 
$^{39}$ \href{https://ror.org/049jf1a25}{National Laboratory of Frascati}, Frascati, Italy, \\ 
$^{40}$ \href{https://ror.org/02an8es95}{National Agency for New Technologies,  Energy and Sustainable Economic Development}, Rome, Italy, \\ 
$^{41}$ \href{https://ror.org/02be6w209}{Sapienza University of Rome}, Rome,Italy, \\ 
$^{42}$ \href{https://ror.org/05j3snm48}{INFN Sezione di Trieste}, Trieste, Italy, \\ 
$^{43}$ \href{https://ror.org/022hq6c49}{INFN Sezione di Bari}, Bari, Italy, \\ 
$^{44}$ \href{https://ror.org/04pmn0e78}{Universidad de Alcal\'a}, Alcal\'a de Henares, Spain, \\ 
$^{45}$ \href{https://ror.org/02k1zhm92}{Laboratori Nazionali del Sud}, Catania, Italy, \\ 
$^{46}$ \href{https://ror.org/00ayhx656}{University of Sussex}, Brighton, United Kingdom, \\ 
%$^{47}$ \href{https://ror.org/05symbg58}{INFN Sezione di Pisa}, Pisa, Italy, \\
$^{47}$ \href{https://ror.org/01tevnk56}{University of Siena}, Siena, Italy,\\
$^{48}$ \href{https://ror.org/042nb2s44}{Massachusetts Institute of Technology}, Cambridge, MA,  United States, \\
$^{49}$ \href{https://ror.org/00bgk9508}{Polytechnic University of Turin}, Turin, Italy, \\ %{NEMO Group, Dipartimento Energia, Politecnico di Torino.\ Corso Duca degli Abruzzi, 24, 10129 Torino, Italy}, \\
$^{50}$ \href{https://ror.org/027ynra39}{University of Bari Aldo Moro}, Bari, Italy, \\%{Universit\'a  di Bari, Dipartimento di Fisica, Via Amendola 173, I-70125 Bari, Italy}, \\
$^{51}$ \href{https://ror.org/013m0ej23}{Perimeter Institute}, Waterloo, ON, Canada, \\
$^{52}$ \href{https://ror.org/02t274463}{University of California, Santa Barbara}, Santa Barbara, CA, United States, \\
$^{53}$ \href{https://ror.org/03dbr7087}{University of Toronto}, Toronto, ON, Canada, \\
$^{54}$ \href{https://ror.org/05n911h24}{Technical University of Darmstadt}, Darmstadt, Germany, \\ %{Institute for Accelerator Science and Electromagnetic Fields, Technische Universit{"a}t Darmstadt, Schlossgartenstr. 8, 64289 Darmstadt, Germany}, \\
$^{55}$ \href{https://ror.org/01hys1667}{LIP---Laboratory of Instrumentation and Experimental Particle Physics}, Lisbon, Portugal, \\%{LIP, Laborat\'{o}rio de Instrumenta\c{c}\~{a}o e F\'{i}sica Experimental de Part\'{i}culas, Lisbon, Portugal}, \\
$^{56}$ \href{https://ror.org/04njjy449}{Universidad de Granada}, Granada, Spain, \\  
$^{57}$ \href{https://ror.org/02vv5y108}{INFN Sezione di Firenze}, Sesto Fiorentino, Italy, \\
$^{58}$ \href{https://ror.org/01x1kqx83}{Bolu Abant Izzet Baysal University}, Bolu, T\"{u}rkiye, \\
$^{59}$ \href{https://ror.org/01kg8sb98}{Indiana University}, Bloomington, IN, United States, \\
$^{61}$ \href{https://ror.org/00twb6c09}{Riga Technical University}, Riga, Latvia, \\
$^{62}$ \href{https://ror.org/00f9tz983}{National Institute for Subatomic Physics}, Amsterdam, Netherlands, \\
$^{63}$ \href{https://ror.org/006hf6230}{University of Twente}, Enschede, Netherlands, \\  
$^{64}$ \href{https://ror.org/04gyf1771}{University of California, Irvine}, Irvine, CA, United States, \\
$^{65}$ \href{https://ror.org/016xsfp80}{Radboud University Nijmegen}, Nijmegen, Netherlands, \\
$^{66}$ \href{https://ror.org/05vf0dg29}{Roma Tre University}, Rome, Italy, \\ %{Universit\`a degli Studi di Roma Tre, Dipartimento di Matematica e Fisica, Via Vasca Navale 84, I-00146 Roma, Rome, Italy}
$^{67}$ \href{https://ror.org/009wnjh50}{INFN Sezione di Roma III}, Rome, Italy, \\ 
$^{68}$ \href{https://ror.org/05xx77y52}{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnologicas}, Madrid, Spain, \\ 
$^{69}$ \href{https://ror.org/00g30e956}{Universit\"at Hamburg}, Hamburg, Germany, \\
$^{70}$ \href{https://ror.org/04t3en479}{Karlsruhe Institute of Technology}, Karlsruhe, Germany, \\ %Karlsruher Institut f{"u}r Technologie (KIT), Kaiserstraße 12, 76131 Karlsruhe, Germany, \\
$^{71}$ \href{https://ror.org/02mpq6x41}{University of Illinois at Chicago}, Chicago, IL,  United States, \\
$^{72}$ \href{https://ror.org/01wv9cn34}{European Spallation Source}, Lund, Sweden, \\
$^{73}$ \href{https://ror.org/01js2sh04}{Deutsches Elektronen-Synchrotron DESY}, Hamburg, Germany, \\
$^{74}$ \href{https://ror.org/0064kty71}{Sun Yat-sen University}, Guangzhou, China, \\ 
$^{75}$ \href{https://ror.org/01an3r305}{University of Pittsburgh}, Pittsburgh, PA, United States, \\
$^{76}$ \href{https://ror.org/020f3ap87}{University of Tennessee at Knoxville}, Knoxville, TN, United States, \\ 
$^{77}$ \href{https://ror.org/03vek6s52}{Harvard University}, Cambridge, MA, United States, \\ 
$^{78}$ \href{https://ror.org/052d0h423}{Max Planck Institute for Nuclear Physics}, Heidelberg, Germany, \\ %Max-Planck-Institut f{\"u}r Kernphysik,  Saupfercheckweg 1, 69117 Heidelberg, Germany, \\
$^{79}$ \href{https://ror.org/041kmwe10}{Imperial College London}, London, United Kingdom, \\
$^{80}$ \href{https://ror.org/02azyry73}{University of Siegen}, Siegen, Germany, \\ 
$^{81}$ \href{https://ror.org/01g5y5k24}{High Energy Accelerator Research Organization}, Tsukuba, Japan, \\ 
$^{82}$ \href{https://ror.org/001tmjg57}{University of Kansas}, Lawrence, KS, United States, \\
$^{83}$ \href{https://ror.org/03angcq70}{University of Birmingham}, Birmingham, United Kingdom, \\
$^{84}$ \href{https://ror.org/04kf25f32}{Shree Guru Gobind Singh Shree Guru Gobind Singh Tricentenary University}, Gurgaon, India, \\
$^{85}$ \href{https://ror.org/00n3w3b69}{University of Strathclyde}, Glasgow, United Kingdom, \\
$^{86}$ \href{https://ror.org/05qwgg493}{Boston University}, Boston, MA, United States, \\
$^{87}$ \href{https://ror.org/017zqws13}{University of Minnesota}, Minneapolis, MN,  United States, \\
$^{88}$ \href{https://ror.org/02v51f717}{Peking University}, Beijing, China, \\ 
$^{89}$ \href{https://ror.org/01y1kjr75}{Nankai University}, Tianjin, China, \\ 
$^{90}$ \href{https://ror.org/008zs3103}{Rice University}, Houston, TX, United States, \\ 
$^{91}$ \href{https://ror.org/02q40pc92}{Fusion for Energy}, Barcelona, Spain, \\ 
$^{92}$ \href{https://ror.org/000e0be47}{Northwestern University}, Evanston, IL, United States, \\ 
$^{93}$ \href{https://ror.org/05gvnxz63}{Argonne National Laboratory}, Lemont, IL, United States, \\ 
$^{94}$ \href{https://ror.org/03c44v465}{Polytechnic University of Bari}, Bari, Italy, \\ 
$^{95}$ \href{https://ror.org/02495e989}{UCLouvain}, Louvain-la-Neuve, Belgium, \\ %{Center for Cosmology, Particle Physics and Phenomenology, Université Catholique de Louvain, Louvain-la-Neuve, Belgium}, \\ 
$^{96}$ \href{https://ror.org/015kcdd40}{INFN  Sezione di Napoli}, Naples, Italy, \\ 
$^{97}$ \href{https://ror.org/041zkgm14}{University of Ferrara}, Ferrara, Italy, \\ 
$^{98}$ \href{https://ror.org/03v8tnc06}{Institute of High Energy Physics}, Beijing, China, \\ 
$^{99}$ \href{https://ror.org/05f0yaq80}{Stockholm University},Stockholm, Sweden, \\ 
$^{100}$ \href{https://ror.org/039bjqg32}{University of Warsaw}, Warsaw, Poland, \\ 
$^{101}$ \href{https://ror.org/048a87296}{Uppsala University}, Uppsala, Sweden, \\ 
$^{102}$ \href{https://ror.org/036jqmy94}{University of Iowa}, Iowa City, IA, United States, \\ 
$^{103}$ \href{https://ror.org/04wn09761}{Universidade Federal do Rio Grande do Norte, Campus Universit\'ario}, Natal, Brazil, \\ 
$^{104}$ \href{https://ror.org/03ad39j10}{University of Pisa}, Pisa, Italy, \\ 
$^{105}$ \href{https://ror.org/02s376052}{École polytechnique fédérale de Lausanne}, Lausanne, Switzerland, \\ 
$^{106}$ \href{https://ror.org/03hasqf61}{Institut de Ciencia de Materials de Barcelona}, Cerdanyola del Vallès, Spain, \\ 
$^{107}$ \href{https://ror.org/008xxew50}{Vrije Universiteit Amsterdam}, Amsterdam, Netherlands, \\ 
$^{108}$ \href{https://ror.org/02mw21745}{Rudjer Boskovic Institute}, Zagreb, Croatia, \\ 
$^{109}$ \href{https://ror.org/02a5smf05}{Cockcroft Institute}, Daresbury, United Kingdom, \\ 
$^{110}$ \href{https://ror.org/05bnh6r87}{Cornell University}, Ithaca, NY, United States, \\ 
$^{111}$ \href{https://ror.org/01n78t774}{Institute of Nuclear Physics, Polish Academy of Sciences}, Krak{\'o}w, Poland, \\ 
$^{112}$ \href{https://ror.org/04wn09761}{Universidade Federal do Rio Grande do Norte, Campus Universit\'ario}, Natal, Brazil, \\ 
$^{113}$ \href{https://ror.org/033003e23}{Tampere University}, Tampere, Finland, \\ 
$^{114}$ \href{https://ror.org/03a62bv60}{University of Malta}, Msida, Malta, \\ 
$^{115}$ {CS\&T, France}, \\ 
$^{116}$ \href{https://ror.org/01swzsf04}{University of Geneva}, Geneva, Switzerland, \\ 
$^{117}$ \href{https://ror.org/03a64bh57}{University of Catania}, Catania, Italy, \\ 
$^{118}$ \href{https://ror.org/03s65by71}{University of California, Santa Cruz}, Santa Cruz, CA, United States, \\ 
$^{119}$ \href{https://ror.org/04d836q62}{TU Wien}, Vienna, Austria, \\ 
$^{120}$ \href{https://ror.org/03m2x1q45}{University of Arizona}, Tucson, AZ, United States, \\ 
$^{121}$ \href{https://ror.org/04c4dkn09}{University of Science and Technology of China}, Hefei, China, \\ 
$^{122}$ {LAPTh, Universit\'{e} Savoie Mont-Blanc et CNRS, Annecy, France}, \\ 
$^{123}$ \href{https://ror.org/0168r3w48}{University of California, San Diego}, La Jolla, CA, United States, \\ 
$^{124}$ \href{https://ror.org/036trcv74}{Nanjing Normal University}, Nanjing, China, \\ 
$^{125}$ \href{https://ror.org/0371hy230}{Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats}, Barcelona, Spain, \\ 
$^{126}$ \href{https://ror.org/01ryk1543}{University of Southampton}, Southampton, United Kingdom, \\ 
$^{127}$ \href{https://ror.org/01wjejq96}{Yonsei University}, Seoul, South Korea, \\ 
$^{128}$ \href{https://ror.org/03x8rhq63}{Institute of Modern Physics}, Lanzhou, China, \\ 
$^{129}$ \href{https://ror.org/05qbk4x57}{University of Chinese Academy of Sciences}, Beijing, China, \\ 
$^{130}$ \href{https://ror.org/017xch102}{Instituto de F\'{\i}sica Corpuscular}, Paterna, Spain%CSIC-Universitat de Val\`encia,   Catedr\'{a}tico Jos\'{e} Beltr\'{a}n 2, E-46980, Paterna, Spain
}
\end{flushleft}

%\newpage

%\thispagestyle{empty}
%\mbox{}
%\vfill


==> AddAuthors/AddAuthors_old3.tex <==
\newpage 
\thispagestyle{empty}

\vskip 10cm
\begin{center}
{\huge\bfseries
Interim report for the \\
International Muon Collider Collaboration (IMCC) }

\end{center}

\vspace{5mm}
{\small
\noindent
Carlotta~Accettura$^{1}$, Simon~Adrian$^{2}$, Rohit~Agarwal$^{3}$, Claudia~Ahdida$^{1}$, Chiara~Aime'$^{4}$, Avni~Aksoy$^{1, 5}$, Gian Luigi~Alberghi$^{6}$, Siobhan~Alden$^{7}$, Nicola~Amapane$^{8, 9}$, David~Amorim$^{1}$, Paolo~Andreetto$^{10}$, Fabio~Anulli$^{11}$, Rob~Appleby$^{12}$, Artur~Apresyan$^{13}$, Pouya~Asadi$^{14}$, Mohammed~Attia Mahmoud$^{15}$, Bernhard~Auchmann$^{16, 1}$, John~Back$^{17}$, Anthony~Badea$^{18}$, Kyu Jung~Bae$^{19}$, E.J.~Bahng$^{20}$, Lorenzo~Balconi$^{21, 22}$, Fabrice~Balli$^{23}$, Laura~Bandiera$^{24}$, Carmelo~Barbagallo$^{1}$, Roger~Barlow$^{25}$, Camilla~Bartoli$^{26}$, Nazar~Bartosik$^{9}$, Emanuela~Barzi$^{13}$, Fabian~Batsch$^{1}$, Matteo~Bauce$^{11}$, Michael~Begel$^{27}$, J. Scott~Berg$^{27}$, Andrea~Bersani$^{28}$, Alessandro~Bertarelli$^{1}$, Francesco~Bertinelli$^{1}$, Alessandro~Bertolin$^{10}$, Pushpalatha~Bhat$^{13}$, Clarissa~Bianchi$^{26}$, Michele~Bianco$^{1}$, William~Bishop$^{17, 29}$, Kevin~Black$^{30}$, Fulvio~Boattini$^{1}$, Alex~Bogacz$^{31}$, Maurizio~Bonesini$^{32}$, Bernardo~Bordini$^{1}$, Patricia~Borges de Sousa$^{1}$, Salvatore~Bottaro$^{33}$, Luca~Bottura$^{1}$, Steven~Boyd$^{17}$, Marco~Breschi$^{26, 6}$, Francesco~Broggi$^{22}$, Matteo~Brunoldi$^{34, 4}$, Xavier~Buffat$^{1}$, Laura~Buonincontri$^{35, 10}$, Philip Nicholas~Burrows$^{36}$, Graeme Campbell~Burt$^{37}$, Dario~Buttazzo$^{38}$, Barbara~Caiffi$^{28}$, Sergio~Calatroni$^{1}$, Marco~Calviani$^{1}$, Simone~Calzaferri$^{34}$, Daniele~Calzolari$^{1}$, Claudio~Cantone$^{39}$, Rodolfo~Capdevilla$^{13}$, Christian~Carli$^{1}$, Carlo~Carrelli$^{40}$, Fausto~Casaburo$^{41, 11, 28}$, Massimo~Casarsa$^{42}$, Luca~Castelli$^{41, 11}$, Maria Gabriella~Catanesi$^{43}$, Lorenzo~Cavallucci$^{26, 6}$, Gianluca~Cavoto$^{41, 11}$, Francesco Giovanni~Celiberto$^{44}$, Luigi~Celona$^{45}$, Alessia~Cemmi$^{40}$, Sergio~Ceravolo$^{39}$, Alessandro~Cerri$^{46, 47, 38}$, Francesco~Cerutti$^{1}$, Gianmario~Cesarini$^{39}$, Cari~Cesarotti$^{48}$, Antoine~Chance$^{23}$, Nikolaos~Charitonidis$^{1}$, mauro~chiesa$^{4}$, Paolo~Chiggiato$^{1}$, Vittoria Ludovica~Ciccarella$^{39, 41}$, Pietro~Cioli Puviani$^{49}$, Anna~Colaleo$^{50, 43}$, Francesco~Colao$^{40}$, Francesco~Collamati$^{11}$, Marco~Costa$^{51}$, Nathaniel~Craig$^{52}$, David~Curtin$^{53}$, Laura~D'Angelo$^{54}$, Giacomo~Da Molin$^{55}$, Heiko~Damerau$^{1}$, Sridhara~Dasu$^{30}$, Jorge~de Blas$^{56}$, Stefania~De Curtis$^{57}$, Herbert~De Gersem$^{54}$, Tommaso~Del Moro$^{41, 40}$, Jean-Pierre~Delahaye$^{1}$, Dmitri~Denisov$^{27}$, Haluk~Denizli$^{58}$, Radovan~Dermisek$^{59}$, Paula~Desiré Valdor$^{1}$, Charlotte~Desponds$^{1}$, Luca~Di Luzio$^{10}$, Elisa~Di Meco$^{39}$, Karri Folan~Di Petrillo$^{18}$, Ilaria~Di Sarcina$^{40}$, Eleonora~Diociaiuti$^{39}$, Tommaso~Dorigo$^{10, 60}$, Karlis~Dreimanis$^{61}$, Tristan~du Pree$^{62, 63}$, Thomas~Edgecock$^{25}$, Siara~Fabbri$^{1}$, Marco~Fabbrichesi$^{42}$, Stefania~Farinon$^{28}$, Guillaume~Ferrand$^{23}$, Jose Antonio~Ferreira Somoza$^{1}$, Max~Fieg$^{64}$, Frank~Filthaut$^{65, 62}$, Patrick~Fox$^{13}$, Roberto~Franceschini$^{66, 67}$, Rui~Franqueira Ximenes$^{1}$, Michele~Gallinaro$^{55}$, Maurice~Garcia-Sciveres$^{3}$, Luis~Garcia-Tabares$^{68}$, Ruben~Gargiulo$^{41}$, Cedric~Garion$^{1}$, Maria Vittoria~Garzelli$^{69}$, Marco~Gast$^{70}$, Cecilia E.~Gerber$^{71}$, Luca~Giambastiani$^{35, 10}$, Alessio~Gianelle$^{10}$, Eliana~Gianfelice-Wendt$^{13}$, Stephen~Gibson$^{7}$, Simone~Gilardoni$^{1}$, Dario Augusto~Giove$^{22}$, Valentina~Giovinco$^{1}$, Alfredo~Glioti$^{23}$, Arkadiusz~Gorzawski$^{72, 1}$, Mario~Greco$^{67}$, Christophe~Grojean$^{73}$, Alexej~Grudiev$^{1}$, Edda~Gschwendtner$^{1}$, Emanuele~Gueli$^{11, 11}$, Nicolas~Guilhaudin$^{1}$, Chengcheng~Han$^{74}$, Tao~Han$^{75}$, John Michael~Hauptman$^{20}$, Matthew~Herndon$^{30}$, Adrian D~Hillier$^{29}$, Micah~Hillman$^{76}$, Tova Ray~Holmes$^{76}$, Samuel~Homiller$^{77}$, Sudip~Jana$^{78}$, Sergo~Jindariani$^{13}$, Sofia~Johannesson$^{72}$, Benjamin~Johnson$^{76}$, Owain Rhodri~Jones$^{1}$, Paul-Bogdan~Jurj$^{79}$, Yonatan~Kahn$^{13}$, Rohan~Kamath$^{79}$, Anna~Kario$^{63}$, Ivan~Karpov$^{1}$, David~Kelliher$^{29}$, Wolfgang~Kilian$^{80}$, Ryuichiro~Kitano$^{81}$, Felix~Kling$^{73}$, Antti~Kolehmainen$^{1}$, K.C.~Kong$^{82}$, Jaap~Kosse$^{16}$, Georgios~Krintiras$^{82}$, Karol~Krizka$^{83}$, Nilanjana~Kumar$^{84}$, Erik~Kvikne$^{1}$, Robert~Kyle$^{85}$, Emanuele~Laface$^{72}$, Kenneth~Lane$^{86}$, Andrea~Latina$^{1}$, Anton~Lechner$^{1}$, Seh Wook~Lee$^{19}$, Junghyun~Lee$^{19}$, Lawrence~Lee$^{76}$, Thibaut~Lefevre$^{1}$, Emanuele~Leonardi$^{11}$, Giuseppe~Lerner$^{1}$, Peiran~Li$^{87}$, Qiang~Li$^{88}$, Tong~Li$^{89}$, Wei~Li$^{90}$, Roberto~Li Voti$^{39}$, Roberto~Li Voti$^{41, 39}$, Mats~Lindroos$^{72}$, Ronald~Lipton$^{13}$, Zhen~Liu$^{47}$, Da~Liu$^{75}$, Miaoyuan~Liu$^{1}$, Alessandra~Lombardi$^{1}$, Shivani~Lomte$^{30}$, Kenneth~Long$^{79, 29}$, Luigi~Longo$^{43}$, José~Lorenzo$^{91}$, Roberto~Losito$^{1}$, Ian~Low$^{92, 93}$, Xianguo~Lu$^{17}$, Donatella~Lucchesi$^{35, 10}$, Tianhuan~Luo$^{3}$, Anna~Lupato$^{35, 10}$, Yang~Ma$^{6}$, Shinji~Machida$^{29}$, Thomas~Madlener$^{73}$, Lorenzo~Magaletti$^{94, 43, 94}$, Marcello~Maggi$^{43}$, Helene~Mainaud Durand$^{1}$, Fabio~Maltoni$^{95, 26, 6}$, Jerzy Mikolaj~Manczak$^{1}$, Marco~Mandurrino$^{9}$, Claude~Marchand$^{23}$, Francesco~Mariani$^{22, 41}$, Stefano~Marin$^{1}$, Samuele~Mariotto$^{21, 22}$, Stewart~Martin-Haugh$^{29}$, Maria Rosaria~Masullo$^{96}$, Giorgio Sebastiano~Mauro$^{45}$, Andrea~Mazzolari$^{24, 97}$, Barbara~Mele$^{11}$, Federico~Meloni$^{73}$, Xiangwei~Meng$^{98}$, Matthias~Mentink$^{1}$, Elias~Metral$^{1}$, Rebecca~Miceli$^{26}$, Natalia~Milas$^{72}$, Abdollah~Mohammadi$^{30}$, Dominik~Moll$^{54}$, Alessandro~Montella$^{99}$, Mauro~Morandin$^{10}$, Marco~Morrone$^{1}$, Tim~Mulder$^{1}$, Riccardo~Musenich$^{28}$, Krzysztof~Mękała$^{100, 73}$, Marco~Nardecchia$^{41, 42}$, Federico~Nardi$^{35}$, David~Neuffer$^{13}$, David~Newbold$^{29}$, Daniel~Novelli$^{28, 41}$, Maja~Olvegård$^{101}$, Yasar~Onel$^{102}$, Domizia~Orestano$^{66, 67}$, John~Osborne$^{1}$, Simon~Otten$^{63}$, Yohan Mauricio~Oviedo Torres$^{103}$, Daniele~Paesani$^{39, 1}$, Simone~Pagan Griso$^{3}$, Davide~Pagani$^{6}$, Kincso~Pal$^{1}$, Mark~Palmer$^{27}$, Alessandra~Pampaloni$^{28}$, Paolo~Panci$^{38, 104}$, Priscilla~Pani$^{73}$, Yannis~Papaphilippou$^{1}$, Rocco~Paparella$^{22}$, Paride~Paradisi$^{35, 10}$, Antonio~Passeri$^{67}$, Nadia~Pastrone$^{9}$, Antonello~Pellecchia$^{43}$, Fulvio~Piccinini$^{4}$, Henryk~Piekarz$^{13}$, Tatiana~Pieloni$^{105}$, Juliette~Plouin$^{23}$, Alfredo~Portone$^{91}$, Karolos~Potamianos$^{17}$, Joséphine~Potdevin$^{105, 1}$, Soren~Prestemon$^{3}$, Teresa~Puig$^{106}$, Ji~Qiang$^{3}$, Lionel~Quettier$^{23}$, Tanjona Radonirina~Rabemananjara$^{107, 62}$, Emilio~Radicioni$^{43}$, Raffaella~Radogna$^{50, 43}$, Ilaria Carmela~Rago$^{11}$, Andris~Ratkus$^{61}$, Elodie~Resseguie$^{3}$, Juergen~Reuter$^{73}$, Pier Luigi~Ribani$^{26}$, Cristina~Riccardi$^{34, 4}$, Stefania~Ricciardi$^{29}$, Tania~Robens$^{108}$, Youri~Robert$^{1}$, Chris~Rogers$^{29}$, Juan~Rojo$^{62, 107}$, Marco~Romagnoni$^{97, 24}$, Kevin~Ronald$^{85, 109}$, Benjamin~Rosser$^{18}$, Carlo~Rossi$^{1}$, Lucio~Rossi$^{21, 22}$, Leo~Rozanov$^{18}$, Maximilian~Ruhdorfer$^{110}$, Richard~Ruiz$^{111}$, Farinaldo~S. Queiroz$^{103, 112}$, Saurabh~Saini$^{46, 1}$, Filippo~Sala$^{26, 6}$, Claudia~Salierno$^{26}$, Tiina~Salmi$^{113}$, Paola~Salvini$^{4, 34}$, Ennio~Salvioni$^{46}$, Nicholas~Sammut$^{114}$, Carlo~Santini$^{22}$, Alessandro~Saputi$^{24}$, Ivano~Sarra$^{39}$, Giuseppe~Scarantino$^{22, 41}$, Hans~Schneider-Muntau$^{115}$, Daniel~Schulte$^{1}$, Jessica~Scifo$^{40}$, Tanaji~Sen$^{13}$, Carmine~Senatore$^{116}$, Abdulkadir~Senol$^{58}$, Daniele~Sertore$^{22}$, Lorenzo~Sestini$^{10}$, Ricardo César~Silva Rêgo$^{103, 112}$, Federica Maria~Simone$^{94, 43}$, Kyriacos~Skoufaris$^{1}$, Gino~Sorbello$^{117, 45}$, Massimo~Sorbi$^{21, 22}$, Stefano~Sorti$^{21, 22}$, Lisa~Soubirou$^{23}$, David~Spataro$^{73}$, Anna~Stamerra$^{50, 43}$, Steinar~Stapnes$^{1}$, Giordon~Stark$^{118}$, Marco~Statera$^{22}$, Bernd Michael~Stechauner$^{119, 1}$, Shufang~Su$^{120}$, Wei~Su$^{74}$, Xiaohu~Sun$^{88}$, Alexei~Sytov$^{24}$, Jian~Tang$^{74}$, Jingyu~Tang$^{121, 98}$, Rebecca~Taylor$^{1}$, Herman~Ten Kate$^{63, 1}$, Pietro~Testoni$^{91}$, Leonard Sebastian~Thiele$^{2, 1}$, Rogelio~Tomas Garcia$^{1}$, Max~Topp-Mugglestone$^{1, 36}$, Toms~Torims$^{61, 1}$, Riccardo~Torre$^{28}$, Luca Tortora~Tortora$^{67, 66}$, Ludovico~Tortora$^{67}$, Sokratis~Trifinopoulos$^{48}$, Sosoho-Abasi~Udongwo$^{2, 1}$, Ilaria~Vai$^{34, 4}$, Riccardo Umberto~Valente$^{22}$, Ursula~van Rienen$^{2}$, Rob~Van Weelderen$^{1}$, Marion~Vanwelde$^{1}$, Gueorgui~Velev$^{13}$, Rosamaria~Venditti$^{50, 43}$, Adam~Vendrasco$^{76}$, Adriano~Verna$^{40}$, Arjan~Verweij$^{1}$, Piet~Verwilligen$^{43}$, Yoxara~Villamzar$^{103}$, Ludovico~Vittorio$^{122}$, Paolo~Vitulo$^{34, 4}$, Isabella~Vojskovic$^{72}$, Dayong~Wang$^{88}$, Lian-Tao~Wang$^{18}$, Xing~Wang$^{123}$, Manfred~Wendt$^{1}$, Markus~Widorski$^{1}$, Mariusz~Wozniak$^{1}$, Yongcheng~Wu$^{124}$, Andrea~Wulzer$^{125, 47}$, Keping~Xie$^{75}$, Yifeng~Yang$^{126}$, Yee Chinn~Yap$^{73}$, Katsuya~Yonehara$^{13}$, Hwi Dong~Yoo$^{127}$, Zhengyun~You$^{74}$, Marco~Zanetti$^{35}$, Angela~Zaza$^{50, 43}$, Liang~Zhang$^{85}$, Ruihu~Zhu$^{128, 129}$, Alexander~Zlobin$^{13}$, Davide~Zuliani$^{35, 10}$, José Francisco~Zurita$^{130}$ }

\vspace{3mm}

\begin{flushleft}
{\em\footnotesize
$^{1}$ {\href{https://ror.org/01ggx4157}{European Organization for Nuclear Research}, Geneva, Switzerland}, \\ 
$^{2}$ {\href{https://ror.org/03zdwsf69}{University of Rostock}, Rostock, Germany}, \\ 
$^{3}$ {\href{https://ror.org/02jbv0t02}{Lawrence Berkeley National Laboratory}, Berkeley, CA, United States}, \\ 
$^{4}$ {\href{https://ror.org/01st30669}{INFN Sezione di Pavia}, Pavia, Italy}, \\ 
$^{5}$ {\href{https://ror.org/01wntqw50}{Ankara University}, Ankara, Türkiye}, \\ 
$^{6}$ {\href{https://ror.org/04j0x0h93}{INFN Sezione di Bologna}, Bologna, Italy}, \\ 
$^{7}$ {\href{https://ror.org/04g2vpn86}{Royal Holloway University of London}, Egham, United Kingdom}, \\ 
$^{8}$ {\href{https://ror.org/048tbm396}{University of Turin}, Turin, Italy}, \\ 
$^{9}$ {\href{https://ror.org/01vj6ck58}{INFN Sezione di Torino}, Turin, Italy}, \\ 
$^{10}$ {\href{https://ror.org/00z34yn88}{INFN Sezione di Padova}, Padua, Italy}, \\ 
$^{11}$ {\href{https://ror.org/05eva6s33}{INFN Sezione di Roma I}, Rome, Italy}, \\ 
$^{12}$ {\href{https://ror.org/027m9bs27}{University of Manchester}, Manchester, United Kingdom}, \\ 
$^{13}$ {\href{https://ror.org/020hgte69}{Fermi National Accelerator Laboratory}, Batavia, IL, United States}, \\ 
$^{14}$ {\href{https://ror.org/0293rh119}{University of Oregon}, Eugene, OR, United States}, \\ 
$^{15}$ {\href{https://ror.org/023gzwx10}{Fayoum University}, Al Fayyūm, Egypt}, \\ 
$^{16}$ {\href{https://ror.org/03eh3y714}{Paul Scherrer Institute}, Villigen, Switzerland}, \\ 
$^{17}$ {\href{https://ror.org/01a77tt86}{University of Warwick}, Coventry, United Kingdom}, \\ 
$^{18}$ {\href{https://ror.org/024mw5h28}{University of Chicago}, Chicago IL, United States America}, \\ 
$^{19}$ {\href{https://ror.org/040c17130}{Kyungpook National University}, Daegu, South Korea}, \\ 
$^{20}$ {\href{https://ror.org/04rswrd78}{Iowa State University}, Ames, IA, United States}, \\ 
$^{21}$ {Universit{"a} degli Studi di Milano, Dipartimento di Fisica, 20133 Milano, Italy}, \\ 
$^{22}$ {Laboratory for Accelerator and Applied Superconductivity, INFN, V. F.lli Cervi 201, 20054 Segrate, Italy}, \\ 
$^{23}$ {IRFU, CEA, Universit\'e Paris-Saclay, France}, \\ 
$^{24}$ {INFN Sezione di Ferrara, via Saragat 1, I-44122 Ferrara, Italy}, \\ 
$^{25}$ {The University of Huddersfield, United Kingdom}, \\ 
$^{26}$ {Universit{\'a} degli Studi di Bologna, Via Zamboni, 33, I-40126 Bologna, Italy}, \\ 
$^{27}$ {Brookhaven National Laboratory, United States}, \\ 
$^{28}$ {INFN sezione di Genova, Via Dodecaneso, 33, I-16146 Genova, Italy}, \\ 
$^{29}$ {ISIS Neutron and Muon Facility, United Kingdom}, \\ 
$^{30}$ {University of Wisconsin-Madison, United States}, \\ 
$^{31}$ {Jefferson Lab, Newport News, Virginia,  United States}, \\ 
$^{32}$ {INFN Sezione di Milano Bicocca, Piazza Scienza 3, I-20123 Milano,Italy}, \\ 
$^{33}$ {School of Physics and Astronomy, Tel-Aviv University, Tel-Aviv 69978, Israel}, \\ 
$^{34}$ {Universit\'a degli Studi di Pavia, Dipartimento di Fisica, via Bassi 6, I-27100, Pavia, Italy}, \\ 
$^{35}$ {Universit\'a degli Studi di Padova, via Marzolo\ 8, 35100 Padova, Italy}, \\ 
$^{36}$ {John Adams Institute, Denys Wilkinson Building, Keble Rd, Oxford OX1 3RH, UK, United Kingdom}, \\ 
$^{37}$ {Lancaster University, Cockcroft Institute, United Kingdom}, \\ 
$^{38}$ {INFN, Sezione di Pisa, Largo Bruno Pontecorvo 3, I-56127 Pisa, Italy}, \\ 
$^{39}$ {INFN Laboratori Nazionali di Frascati, Via Enrico Fermi 54 I-00044, Frascati, Italy}, \\ 
$^{40}$ {ENEA - Italian National Agency for New Technologies,  Energy and Sustainable Economic Development, Italy}, \\ 
$^{41}$ {Universit\'a di Roma Sapienza, I-00185 Roma,Italy}, \\ 
$^{42}$ {INFN Sezione di Trieste, Trieste, Italy}, \\ 
$^{43}$ {INFN Sezione di Bari,  Via Orabona 4, I-70125 Bari, Italy}, \\ 
$^{44}$ {Universidad de Alcal\'a (UAH), Departamento de F\'isica y Matem\'aticas, E-28805 Alcal\'a de Henares, Madrid, Spain}, \\ 
$^{45}$ {INFN Laboratori Nazionali del Sud, Via Santa Sofia, 62, I-95123 Catania, Italy}, \\ 
$^{46}$ {University of Sussex, United Kingdom}, \\ 
$^{47}$ {University of Minnesota, United States}, \\ 
$^{48}$ {Massachusetts Institute of Technology, 77 Massachusetts Ave, 02139 Cambridge, MA,  United States}, \\ 
$^{49}$ {NEMO Group, Dipartimento Energia, Politecnico di Torino, Corso Duca degli Abruzzi 24, I-10129 Torino, Italy}, \\ 
$^{50}$ {Universit\'a  di Bari, Dipartimento di Fisica, Via Amendola 173, I-70125 Bari, Italy}, \\ 
$^{51}$ {Perimeter Institute for Theoretical Physics, 31 Caroline St N, Waterloo, ON N2L 2Y5, Canada}, \\ 
$^{52}$ {University of California, Santa Barbara, CA  United States}, \\ 
$^{53}$ {Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}, \\ 
$^{54}$ {Institute for Accelerator Science and Electromagnetic Fields, Technische Universit{"a}t Darmstadt, Schlossgartenstr. 8, 64289 Darmstadt, Germany}, \\ 
$^{55}$ {LIP, Laborat\'{o}rio de Instrumenta\c{c}\~{a}o e F\'{i}sica Experimental de Part\'{i}culas, Lisbon, Portugal}, \\ 
$^{56}$ {Departamento de Física Teórica y del Cosmos, Universidad de Granada  Campus de Fuentenueva, E-18071 Granada, Spain}, \\ 
$^{57}$ {INFN Sezione di Firenze, Via G. Sansone 1, I-50019 Sesto Fiorentino, Firenze, Italy}, \\ 
$^{58}$ {Department of Physics, Bolu Abant Izzet Baysal University, 14280, Bolu, T\"{u}rkiye, Türkiye}, \\ 
$^{59}$ {Department of Physics, Indiana University, Bloomington, IN, 47403, United States}, \\ 
$^{60}$ {Luleå University of Technology, Sweden}, \\ 
$^{61}$ {Institute of Particle Physics and Accelerator Technologies, Faculty of Natural Sciences and Technology,  Riga Technical University, 6A Kipsalas Street, Riga LV-1048, Latvia}, \\ 
$^{62}$ {Nikhef - National Institute for Subatomic Physics, Science Park 105, 1098 XG Amsterdam, The Netherlands}, \\ 
$^{63}$ {UTWENTE, Netherlands}, \\ 
$^{64}$ {Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, United States}, \\ 
$^{65}$ {Radboud University, Heyendaalseweg 135, 6525 AJ, Nijmegen, The Netherlands}, \\ 
$^{66}$ {Universit\`a degli Studi di Roma Tre, Dipartimento di Matematica e Fisica, Via Vasca Navale 84, I-00146 Roma, Rome, Italy}, \\ 
$^{67}$ {INFN, Sezione di Roma Tre, Italy}, \\ 
$^{68}$ {CIEMAT, Spain}, \\ 
$^{69}$ {II Institut f\"ur Theoretische Physik, Universit\"at Hamburg, Luruper Chaussee 149, 22761 Hamburg, Germany}, \\ 
$^{70}$ {Karlsruher Institut f{"u}r Technologie (KIT), Kaiserstraße 12, 76131 Karlsruhe, Germany}, \\ 
$^{71}$ {University of Illinois Chicago, Department of Physics MC 273 SES 2236, 845 W.\ Taylor St.\, Chicago, IL.\ 60607,  United States}, \\ 
$^{72}$ {ESS, European Spallation Source, Lund, Sweden}, \\ 
$^{73}$ {Deutsches Elektronen-Synchrotron DESY, Notkestr.\ 85, 22607 Hamburg, Germany}, \\ 
$^{74}$ {Sun Yat-Sen University, China}, \\ 
$^{75}$ {University of Pittsburgh, Pittsburgh, PA 15260,  United States}, \\ 
$^{76}$ {University of Tennessee, Knoxville, United States}, \\ 
$^{77}$ {Department of Physics, Harvard University, Cambridge, MA 02138,  United States}, \\ 
$^{78}$ {Max-Planck-Institut f{\"u}r Kernphysik,  Saupfercheckweg 1, 69117 Heidelberg, Germany}, \\ 
$^{79}$ {Department of Physics, Blackett Laboratory, Imperial College, London, SW7 2AZ, United Kingdom}, \\ 
$^{80}$ {Center for Particle Physics Siegen, University of Siegen, 57068 Siegen, Germany}, \\ 
$^{81}$ {KEK Theory Center, Tsukuba 305-0801, Japan}, \\ 
$^{82}$ {Department of Physics and Astronomy, University of Kansas, Lawrence, KS 66045 United States}, \\ 
$^{83}$ {School of Physics and Astronomy, University of Birmingham, Edgbaston, Birmingham B15 2TT, United Kingdom}, \\ 
$^{84}$ {Shree Guru Gobind Singh Shree Guru Gobind Singh Tricentenary University, Gurugram-Badii Road, Gurugram-122505, India}, \\ 
$^{85}$ {University of Strathclyde, 199 Cathedral Street, Glasgow, Scotland , United Kingdom}, \\ 
$^{86}$ {Department of Physics, Boston University, 590 Commonwealth Avenue, Boston, MA 02215, United States}, \\ 
$^{87}$ {School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455,  United States}, \\ 
$^{88}$ {Peking University, China}, \\ 
$^{89}$ {School of Physics, Nankai University, Tianjin 300071, China}, \\ 
$^{90}$ {Rice University, 6100 Main St., Houston, TX 77005, United States}, \\ 
$^{91}$ {Fusion for Energy, Carrer Josep Pla 2, B3, 08019 Barcelona, Spain}, \\ 
$^{92}$ {Department of Physics and Astronomy, Northwestern University, Evanston, Illinois 60208, United States}, \\ 
$^{93}$ {ANL, High Energy Physics Division, Argonne National Laboratory, United States}, \\ 
$^{94}$ {Politecnico di Bari, Italy}, \\ 
$^{95}$ {Center for Cosmology, Particle Physics and Phenomenology, Université Catholique de Louvain, Louvain-la-Neuve, Belgium}, \\ 
$^{96}$ {INFN  Sezione di Napoli, Napoli, Compl. Univ. MSA ed.6, 80126, Napoli, Italy}, \\ 
$^{97}$ {Department of Physics and Earth Science, University of Ferrara, Via Saragat 1, 44122 Ferrara, Italy}, \\ 
$^{98}$ { Institute of High Energy Physics (IHEP) , Chinese Academy of Sciences (CAS)\ 19B Yuquan Road, Shijingshan District, Beijing, 100049, China}, \\ 
$^{99}$ {Department of Physics, Stockholm University\ AlbaNova University Center, 106 91 Stockholm, Sweden}, \\ 
$^{100}$ {Faculty of Physics, University of Warsaw, Pasteura 5, 02-093 Warsaw, Poland}, \\ 
$^{101}$ {Uppsala University, Box 256, 751 05 Uppsala, Sweden}, \\ 
$^{102}$ {University of Iowa, Iowa City, IA 52242, United States}, \\ 
$^{103}$ {International Institute of Physics, Universidade Federal do Rio Grande do Norte, Campus Universit\'ario, Lagoa Nova, Natal-RN 59078-970, Brazil}, \\ 
$^{104}$ {Univesit\'{a} di Pisa, Dipartimento di Fisica, Largo Bruno Pontecorvo 3, I-56127 Pisa, Italy}, \\ 
$^{105}$ {École polytechnique fédérale de Lausanne, Switzerland}, \\ 
$^{106}$ {Institut de Ciencia de Materials de Barcelona, CSIC, Campus UAB, 08193 Bellaterra, Spain}, \\ 
$^{107}$ {Vrije Universiteit, Netherlands}, \\ 
$^{108}$ {Institute Rudjer Boskovic, Croatia}, \\ 
$^{109}$ {The Cockcroft Institute, United Kingdom}, \\ 
$^{110}$ {Laboratory for Elementary Particle Physics, Cornell University, Ithaca, NY 14853,  United States}, \\ 
$^{111}$ {Institute of Nuclear Physics, Polish Academy of Sciences {\rm (IFJ PAN)}, ul. Radzikowskiego, Krak{\'o}w, 31-342, Poland}, \\ 
$^{112}$ {Universidade Federal do Rio Grande do Norte, Brazil}, \\ 
$^{113}$ {Tampere University, 33720 Tampere, Finland}, \\ 
$^{114}$ {University of Malta, Msida, Malta}, \\ 
$^{115}$ {CS\&T, France}, \\ 
$^{116}$ {Universit\'e de Gen\`eve, Switzerland}, \\ 
$^{117}$ {Universit\`a di Catania, DIEEI, Via Santa Sofia 64, I-95123 Catania, Italy}, \\ 
$^{118}$ {Santa Cruz Institute for Particle Physics, University of California Santa Cruz, Santa Cruz, CA,  United States}, \\ 
$^{119}$ {TU Wien, 1040 Vienna, Austria}, \\ 
$^{120}$ {University of Arizona, United States}, \\ 
$^{121}$ {University of Science and Technology of China}, \\ 
$^{122}$ {LAPTh, Universit\'{e} Savoie Mont-Blanc et CNRS, Annecy, France}, \\ 
$^{123}$ {Department of Physics and Astronomy, University of California, San Diego, 9500 Gilman Drive, La Jolla, CA-92093,  United States}, \\ 
$^{124}$ {Department of Physics and Institute of Theoretical Physics, Nanjing Normal University, Nanjing, 210023, China}, \\ 
$^{125}$ {ICREA, Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, Passeig de Llu\'{\i}s Companys 23, 08010 Barcelona, Spain}, \\ 
$^{126}$ {School of Engineering, Faculty of Engineering and Physical Sciences, University of Southampton, Southampton SO171BJ, UK, United Kingdom}, \\ 
$^{127}$ {Department of Physics, Yonsei University, Seoul, Republic of Korea, South Korea}, \\ 
$^{128}$ {Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou 730000, China}, \\ 
$^{129}$ {University of Chinese Academy of Sciences, China}, \\ 
$^{130}$ {Instituto de F\'{\i}sica Corpuscular, CSIC-Universitat de Val\`encia,   Catedr\'{a}tico Jos\'{e} Beltr\'{a}n 2, E-46980, Paterna, Spain}}
\end{flushleft}

%\newpage

%\thispagestyle{empty}
%\mbox{}
%\vfill


==> Chapters/10-CollaborationDevelopment/Author10.tex <==
% !TeX root = ..\CYR2019.tex
\section{Development of the collaboration
% (S. Stapnes, N. Pastrone, D. Schulte, M. Palmer, S. Jindariani, D. Stratakis)
}

%\begin{flushleft}
%\blfootnote{
%This chapter should be cited as:
%Overview of radiation effects on detector systems, Eds.~I.~Dawson, M.~Moll, %F.~Faccio, A.~Weidberg, 
%DOI:~\href{https://doi.org/10.23730/CYRSP-2024-XXX.\thepage}{10.23730/CYRSP-%2024-XXX.\thepage},  in:
%Proceedings of the Joint Universities Accelerator School (JUAS): Courses and %exercises, E. M\'{e}tral (ed.),
%\\CERN Yellow Reports: School Proceedings, CERN-2024-XXX,
%DOI:~\href{https://doi.org/10.23730/CYRSP-2024-XXX}{10.23730/CYRSP-2024-XXX}%,  p. \thepage.
%\\ \copyright\space CERN, 2024. Published by CERN under the 
%\href{http://creativecommons.org/licenses/by/4.0/}{Creative Commons %Attribution 4.0 license}.
%}
%\end{flushleft}

\label{sec:Section10}

The International Muon Collider Collaboration (IMCC) was initiated in 2020 following the recommendations of the European Strategy for Particle Physics (ESPP).  The Muon Collider Study (MuC) covers the accelerator complex, detectors and physics for a future muon collider. In 2023 European Commission support was obtained for a Design Study of a muon collider (MuCol). This project started 1.3.2023, with work-packages aligned with the overall Muon Collider Studies.
Another important development have been the preparation and studied made for the US Snowmass and P5 processes 2021-23, which have focused the muon collider community towards common physics~\cite{c:white1}, detector and accelerator studies for a future muon collider.

\subsection{Muon collider as part of the LDG roadmap}

The muon collider collaboration, the muon beam panel of the Laboratory Directors Group (LDG) and the Snowmass process in the US assessed the muon collider challenges and concluded that the concept is less mature than linear colliders and that important challenges have to be addressed. However, no insurmountable obstacles were identified. 

Past work, in particular within the US Muon Accelerator Programme (MAP)~\cite{map}, has demonstrated several key MuC technologies and concepts, and gives confidence that the overall concept is viable. Component designs and technologies have been developed that can cool the initially diffuse beam and accelerate it to multi-TeV energy on a time scale compatible with the muon lifetime. However, a fully integrated
design has yet to be developed and further development and demonstration of
technology is required. In order to enable the next European Strategy for
Particle Physics update and other international 
strategy processes to judge the scientific justification of a full
Conceptual Design Report (CDR) and a demonstration programme, the design and
potential performance of the facility must be developed with some urgency.

The LDG roadmap  report~\cite{ldg} identifies a set of key studies that have to be addressed in the coming years to prepare the grounds for a Conceptual Design Report (CDR) and demonstrator programme for a muon collider, namely:
\begin{itemize}
\item The {\bf physics potential} has to be further explored; 10~TeV is uncharted territory. 
\item The {\bf environmental impact} must be minimised and at least one {\bf potential site} for the collider identified. 
\item The impact of {\bf beam induced background} in the detector might limit the 
physics reach and has to be minimised. 
\item The muon {\bf acceleration and collision} systems become more demanding at higher energies and are the most important cost and power consumption drivers. The concept and technologies have to be developed beyond what MAP has considered. 
\item The muon {\bf production and cooling system} are challenging novel systems and call for development and optimisation beyond the MAP designs.
\end{itemize}

The muon collider collaboration aims to perform these studies in time for the next Update of the European Strategy for Particle Physics. 
Three main deliverables are foreseen:
\begin{itemize}
\item a Project Evaluation Report that assesses the muon collider potential;
\item an R\&D Plan that describes a path towards the collider;
\item an Interim Report early 2024 that documents progress and allows the wider community to be updated on the concept and to give feedback to the collaboration.
\end{itemize}

As mentioned the muon collider collaboration envisages to study the 10\,TeV option, and also
explore lower and higher energy options, e.g.~a 3\,TeV option as a step toward
10\,TeV. The details of the required work and the required resources are detailed in the LDG roadmap report~\cite{ldg}. 
%While important initial resources have been available, additional resources have recently become available via an EU co-funded design study that started in March 2023. This has also allowed to secure corresponding resources from key partners. However, the current total is not yet sufficient to fully achieve the goals above and additional resources are being sough across the collaboration. 

\subsection {The International Muon Collider Collaboration}
A Memorandum of Cooperation (MoC) for the IMCC has been drawn up and the collaboration is rapidly growing. 
The formal structure of the collaboration, as shown in Fig.~\ref{f:governance} consists of the following main bodies: 
\begin{itemize}
\item International Collaboration Board (ICB):
The ICB role is to provide a forum for participants to examine ongoing activities,
assure appropriate, well directed use of contributions and ensure
a balanced portfolio of engagements.
The chair of the ICB is elected by its members (simple majority).
The ICB consists of one representative of each participating institute that has signed the MoC. The ICB has been active since October 2022. 
\item Steering Board (SB):
The SB oversees the execution of the Muon Collider Study by assessing the progress, resource usage and providing guidance.
The SB reports to the LDG in Europe and to similar regional supervising organisations in other regions as required.
The SG is active and operational since Spring 2023. 
\item International Advisory Committee (IAC): The mandate of the International Advisory Committee is to review the
scientific and technical progress of the Study. This body is in the process of being set up.
\item Coordination Committee (CC): The CC performs the overall coordination and execution of the Muon Collider Study.
It is chaired by the Study Leader. This body consists of experts across the main working areas of the collaboration and is very active. It provides the daily guidance of the study. 
\end{itemize}


\begin{figure}
\centerline{\includegraphics[width=12cm]{Chapters/10-CollaborationDevelopment/Figures/governance-june22.pdf}}
\caption{Organigram of the Muon Collider Study governance structure.}
\label{f:governance}
\end{figure}

The Study Leader is proposed by the host organization, and endorsed by the ICB. The Study Leader was appointed in 2022 and has led the work to build up the collaboration and activities since then.

\subsection {MuCol}

IMCC successfully applied for an EU cofunded design study (named MuCol)~\cite{mucol}. The project started 1.3.2023. The total co-funding of MuCol amounts to 3\,MEUR, provided by
the European Commission, the UK and Switzerland. In the design study, CERN only receives limited contributions for
administrative support and travel, but has, in support of the successful Design Study bid, increased its contribution to the muon collider study.

The design study is fully integrated in the overall muon collaboration. The technical meetings and leaders are in common and governance and management will also be synchronised. The organisation is shown in Fig.~\ref{f:MuColwp}.
Important activities in the collaboration, directly supported by the MuCol work-packages listed below, are:
\begin{itemize}
\item {\bf Physics and Detector Requirements} provides the link to the
physics and detector studies.Based on feedback from
the physics community, it will provide feedback and guidance to the
accelerator design. 
\item {\bf The Proton Complex} addresses the key challenge of the
accumulation of the protons in very high-charge bunches, by addressing in
details the proton complex design, and provides the basic parameters of
the complex and the characteristics of the beam impacting on the production
target.
\item {\bf The Muon Production and Cooling} addresses the production of the
muons by the proton beam hitting a target and the subsequent cooling,
including some of the specific technologies, such as for the production target
and the absorbers that reduce the beam phase space volume.
\item {\bf The High-energy Complex} studyies the acceleration and collision complex of the muons.
\item {\bf Radio Frequency Systems} addresses the Radio Frequency (RF)
systems of the muon cooling ensuring coherence in frequency choice and
synchronization among the various stages. It contributes to sustainability studies by its work on high efficiency RF Power sources.
\item {\bf Magnet Systems} will establish a complete inventory of the necessary
magnets to optimize and standardise the design, and address the most critical
ones. In particular it focuses on the solenoids of the muon production and
cooling, which are specific to the muon collider, and the fast-ramping magnet
system, which have ambitious requirements on power flow and power efficiency
and limits the energy reach of the collider.
\item {\bf Cooling Cell Integration} addresses the design of the muon
cooling cell, which is a unique and novel design and that faces integration
challenges.
\end{itemize}

\begin{figure}
\centerline{\includegraphics[width=10cm]{Chapters/10-CollaborationDevelopment/Figures/MuCol_WP.png}}
\caption{The MuCol workpackages and their interactions.}
\label{f:MuColwp}
\end{figure}


\subsection {Extending the collaboration---US plans}

More than 60 groups are currently involved in the Muon Collider studies. 
The US groups are very active and in leading roles in the IMCC, e.g.\, in the Coordination Committee and the Publications and Speakers Committee, even though in several cases the formal MoC signatures and ramp up the efforts will need to wait for the forthcoming implementation planning of the P5 recommendations.

The collaboration plans to revise both the organisation and the workplan together with  US colleagues. This will also impact the work programme laid out in this report. In particular, the ambition of the US to host such a facility strengthens the motivation for R\&D and demonstrator planning at a fast pace.

The collaboration also plans to attempt further strengthening other regions' participation during this process. There is at this moment an important potential for substantial expansion of the collaboration, resources and efforts in Asia, and several European countries, Canada and South America.  

\subsection {Brief summary}
An international muon collider collaboration, currently hosted by CERN, has been formed. A successful EU Design Study bid has been made. With involvement of the global community a concise set of work-packages has been developed for the LDG accelerator R\&D roadmap. US groups are already part of the muon collider effort, however the recent P5 report opens for a substantial increased US effort over the coming years.  The programme provides an excellent basis for the global collaboration and planning of future work towards a multi-TeV muon collider. The project continues to make important progress with a growing collaboration and community enthusiastically supporting it. 


\begin{thebibliography}{99}

\bibitem{ldg}
  European Large National Laboratories Directors Group (LDG), European Strategy for Particle Physics---Accelerator R\&D Roadmap, CERN-2022-001 (CERN, Geneva, 2022), \href{http://dx.doi.org/10.23731/CYRM-2022-001}{doi:10.23731/CYRM-2022-001}.

\bibitem{c:white1}
  C. Aimé {\it et al.}, Muon Collider physics summary, FERMILAB-PUB-22-377-PPD (Fermilab,  Batavia, IL, 2022), \href{https://doi.org/10.48550/arXiv.2203.07256}{doi:10.48550/arXiv.2203.07256}. 

\bibitem{mucol}
MuCol - A design study for a Muon Collider complex at 10 TeV center of mass, \href{https://mucol.web.cern.ch}{https://mucol.web.cern.ch},  last accessed 15 May 2024.

\bibitem{map}
    M.\,A.\,Palmer and K.\,Long (eds.), Muon accelerators for particle physics (MUON), \textit{JINST special issue} (2016--2021), \href{https://iopscience.iop.org/journal/1748-0221/page/extraproc46}{Article collection}; Muon accelerator program (MAP), \href{http://map.fnal.gov}{http://map.fnal.gov} (restricted access), \href{https://web.archive.org/web/20210505140022/http://map.fnal.gov/}{archived version 5 May 2021} (free access).

\end{thebibliography}

%\subsection{Redundant text}

%The following text is leftover from somewhere and someone. It is not a part of secton 10. 


%\noindent
%Muon colliders can in principle reach the highest lepton collision energies with the required luminosity for affordable cost and power consumption. This allows unprecedented exploration in direct searches of new heavy states and high-precision tests of Standard Model phenomena. The required luminosity increase with the square of the energy can in principle be provided with a constant beam current, i.e. with an only linear increase in the beam power with energy. The full physics potential at high energies remains to be quantified. But first explorations are encouraging. For example, the number of produced Higgs bosons will allow to measure its couplings to fermions and bosons with an unprecedented precision. Moreover, a collider with a centre-of-mass energy in the range of $\sqrt{s} \simeq 10$\,TeV  or above and with a luminosity of the order of $10^{35}$ cm$^{−2}$ s$^{−1}$  will have a very high double and triple Higgs-boson production rate, which will allow to directly measure the parameters of trilinear and quadrilinear self-couplings, enabling the precise determination of the Higgs boson potential. An important concern is the impact of the high background level induced by the muon beam decays. This has to be studied in detail, including potential mitigation methods. A recent exploratory study is encouraging and demonstrated that the measurement of $\mu^{+}\mu^{-}$ → $H \nu \overline{\nu} $ → $b \overline{b} \nu \overline{\nu}$ process is feasible in this harsh environment, with a precision on $\sigma(\nu \nu H)$·BR($H$ → $b \overline{b}$) at the level of less than 1$\%$ at $\sqrt{s} = 3$\,TeV, competitive to other proposed machines. 

%Important progress has been made on the concept of such a collider and on individual hardware components but further development and innovation is required to bring the technology to a maturity level that allows reliable predictions of the performance, cost, power consumption and risk. We propose to form a collaboration and develop a muon collider design in the range of 3\,TeV centre-of-mass energy and a luminosity of $L$ = 1.8 × 10$^{34}$ cm$^{−2}$ s$^{−1}$ and explore a potential second stage, tentatively at 14\,TeV and $L$ = 4 × 10$^{35}$ cm$^{−2}$ s$^{−1}$. Lower energy stages might be considered if they have not been covered by other projects in due time.
%Given the current level of maturity, the proton-driven muon source would be the baseline and the positron-driven source would be developed as the option that could have a lower beam current and mitigate radiation limitations at higher energies from muon beam decays.
%The technically limited plan foresees a four year period to establish a baseline design, which allows to evaluate the risk and cost scale of the project and defines the required test facility or facilities as a basis for further decisions. This would be followed by six years of construction and operation of the facility and the optimisation of the collider design. The results of this phase will allow to decide on committing to the project in which case a technical design could be developed in the following four years.

%In addition to the technical challenges, two main limitations exist for the energy reach of the muon collider. The first is given by the cost and site requirements. Therefore an optimisation for cost and footprint is instrumental and has to be an important consideration during the design phase. The second limitation is given by the ability to achieve the required luminosity with an affordable power consumption and cost.
%The level of luminosity required for different energy reach and purposes may vary. The current baseline is to aim for $L$ $\simeq$ $(\frac{\sqrt{s}}{10 \text{TeV}})^{2}$ × 2 × 10$^{35}$ cm$^{−2}$ s$^{−1}$. The muon collider could be implemented in energy stages to limit the cost and risk of each stage, while still providing excellent physics. The choice of stages will also depend on future findings of the HL-LHC and other relevant colliders.
%To get starget, first considerations yielded the following tentative conclusions that will be reviewed as the work progresses:
%\begin{itemize}
%
%\item {The design effort should focus on an initial energy stage at 3\,TeV with a luminosity of 1.8~×~10$^{34}$~cm$^{−2}$~s$^{−1}$. This matches the maximum energy of CLIC and is a good point to compare the merits of the approaches. This energy also appears consistent with the use of the LHC tunnel for the muon accelerator, the optimum collider ring circumference would be smaller.}
%\item {A second stage will be explored at higher energies, i.e. tentatively 14\,TeV with a luminosity of 4~×~10$^{35}$~cm$^{−2}$~s$^{−1}$ where the discovery potential superseedes any other future collider evaluated at the moment.}
%\item {A dedicated design effort for a muon collider at lower energies (below 3\,TeV) is feasible, but requires dedicated additional studies. Currently no studies are foreseen but this will have to be reviewed as the progress and choices of other projects become clearer.}
%\end{itemize}

%Successful implementation of a muon collider is based on a wide range of cutting edge technologies. In particular, key technologies are:
%\begin{itemize}
%
%\item {High field, robust and cost-effective superconducting magnets for the muon production, cooling, acceleration and collision. High-temperature superconductors would be an ideal option.}
%\item {High-gradient and robust normal-conducting RF to minimise muon losses during cooling.}
%\item {Fast ramping normalconducting, superferric or superconducting magnets that can be used in a rapid cycling synchrotron to accelerate the muons.}
%\item {Efficient, high-gradient superconducting RF to minimise power consumption and muon losses during acceleration.}
%\item {Efficient cryogenics systems to minimise the power consumption of the superconducting components and minimise the impact of beam losses.}
%\item {Robust materials for muon cooling and also collimation and machine protection.}
%\item {Advanced detector concepts and technologies to deal with the background induced by the muon beams.}
%\item {Other accelerator technologies including high-performance, compact vacuum systems to minimise magnet aperture and cost as well as fast, robust, high-resolution instrumentation.}
%\end{itemize}

%Laboratories in Europe and world-wide have important expertise in these areas and could further develop these technologies to enable a muon collider and push its performance reach. The formation of a collaboration to initiate and coordinate a development programme appears indispensible. In the first phase of the programme, the development of the baseline, this effort would largely draw on the experience while in later stages it will focus more on prototyping.
%At least one test facility will be required to develop the muon collider concept to address the most critical challenges. The production of a high quality muon beam will be key and most likely the lion share of this effort. The collaboration will have to develop the experimental beam programme and its implementation drawing on the expertise of the contributing laboratories.

%The reuse of existing CERN infrastructure can have a significant impact on the cost and risk of a muon collider. Hence, the potential to use and modify the existing proton installations and related instrastructure should be investigated as well as the reuse of existing buildings, tunnels and services.
%The muon source requires an important proton beam current, and one can consider upgrading the existing proton infrastructure to meet the requirements. Other equipment could be used for the new complex, e.g.~existing cooling plants could potentially be used for the accelerator and collider rings.
%The main reuse of tunnels is for the accelerator and for the collider ring. The latter should be as small as possible to maximise luminosity. The former will be longer and has less stringent requirements on the length. It is therefore expected to profit more from existing tunnels. Tentative estimates indicate that the LHC tunnel might be adapted to house the accelerator ring for a 3\,TeV collider, while a purpose-built, smaller collider ring would be preferred for this option.
%An important consideration for the tunnels is the neutrino radiation. It can come from the arcs or more important from the straight insertions. Civil engineering studies should identify the locations of highest radiation. It may be possible to improve the situation by acquiring the surface sites corresponding to the highest radiation. A detailed study should be performed of the potential mitigation of the radiation from the straights by a special optics design. One can envisage to bend the beam in the vertical plane using alternating sets of dipoles to produce a wave-like orbit. This can dilute the radiation. More advanced concepts should be considered.

%The rest mass of the muons is $m_{\mu 0}$ = 105.7 MeV/$\text{c}^{2}$ and its lifetime in the reference frame is $\tau_{\mu 0}$~=~2.2~$\mu$s. The 4 main challenges are linked to the fact that muons are decaying particles \cite{IMCC webpage} \cite{MAP} \cite{MICE} \cite{LEMMA} 
%\begin{itemize}
%
%\item {Muon production.}
%\item {Fast muon cooling.}
%\item {Fast acceleration.}
%\item {Neutrino radiation.}
%\end{itemize}

%Thanks to special relativity, the muons lifetime is longer in the laboratory frame and it is given by $\tau_{\mu}$~=~$\tau_{\mu 0} \gamma$, where $\gamma$ is the relativistic Lorentz mass factor. For the highest muons energy considered here, i.e. 7\,TeV (for a collider with a centre-of-mass energy of 14\,TeV), the muons lifetime becomes $\sim$~150\,ms. Therefore, everything needs to be done very quickly with muons. 

%The full chain is depicted in Fig.~\ref{fig:FullChain}. The goal of the Proton Driver is to generate a high (few MW) beam power, short (1-2\,ns) bunch length, low (5\,Hz) repetition rate on a target. In the Front End, pions are produced, decaying in muons which needs to be captured. The muons need then to be (rapidly) cooled and therefore only ionisation cooling in matter can be used. This is done in a sequence of absorbers and RF cavities in high magnetic fields. The final cooling is limited by the highest achievable magnetic field for solenoid of $\sim$ 30\,T (could be solved if the magnetic field could be increased to $\sim$ 50\,T). Then, the muons need to be accelerated from a momentum of $\sim$ 0.2\,GeV/c to the TeV/c scale. This means, as it will be computed below, that the RF gradient for the muon survival is in the MV/m range. In synchrotrons, this means that the dB/dt needs to be in the few kT/s range. Finally, the main worry in the collider is the neutrino radiation which needs to be mitigated, in particular for the highest energies. 

%\begin{figure}[h]
%  \begin{center}

%  \includegraphics[width=0.9\textwidth]{Chapters/10-CollaborationDevelopment/Figures/PictureOfTheFullChain.png}
%  \end{center}
%\caption{The full chain of accelerators of the IMCC (deduced from MAP)}
%\label{fig:FullChain}
%\end{figure}

%The derivation of the required accelerating gradient can be done as follows. When the energy is constant (i.e. $\tau_{\mu}$~=~$\tau_{\mu 0} \gamma$ is constant), the survival rate of the muons is given by 

%\begin{equation}
%\frac{N(t)}{N_{0}} = e^{-\frac{t}{\tau_{\mu}}},
%\label{eq:MuonSurvivalRateConstant}
%\end{equation}

%while when the energy is changing it is given by 

%\begin{equation}
%\frac{N(t)}{N_{0}} = e^{-\frac{1}{\tau_{\mu 0}} \int^{t}_{0}\frac{du}{\gamma(u)}}.
%\label{eq:MuonSurvivalRateAcceleration}
%\end{equation}

%Assuming a linear acceleration ramp for the latter case, the relativistic Lorentz mass factor can be written 

%\begin{equation}
%\gamma(t) = \gamma_1 + \frac{\gamma_2-\gamma_1}{\tau_{acc}} t,
%\label{eq:LorentzMassFactorAcceleration}
%\end{equation}

%and therefore the muons survival rate becomes

%\begin{equation}
%\frac{N_2}{N_1} = \left(\frac{\gamma_2}{\gamma_1}\right)^{-\frac{1}{\tau_{\mu 0}}(\frac{\tau_{acc}}{\gamma_2-\gamma_1})}. 
%\label{eq:MuonSurvivalRateAcceleration2}
%\end{equation}

%The required average accelerating gradient can be expressed as a function of the energy change as follows. Starting from the relation between the total energy and the rest energy, $E(t)=\gamma(t) E_0$, one can write 

%\begin{equation}
%E(t) = E_1 + \frac{E_2-E_1}{\tau_{acc}} t,
%\label{eq:EnergyVariationDuringAcceleration}
%\end{equation}

%and therefore $\Delta E(t) = \frac{E_2-E_1}{\tau_{acc}} t$. Using the fact that the muon speed, at relatively high energy, is approximated by $v = c = \frac{L}{t}$, one can write the required average accelerating gradient as 

%\begin{equation}
%G_{acc}(t) = \frac{\Delta E(t)}{e L} = \frac{E_2-E_1}{e c \tau_{acc}}.
%\label{eq:RequiredAverageAccelGradient}
%\end{equation}

%Finally, using Eq.~\ref{eq:MuonSurvivalRateAcceleration2}, one can show that 

%\begin{equation}
%\tau_{acc} = - \tau_{\mu 0} (\gamma_2-\gamma_1) \frac{\ln{\frac{N_2}{N_1}}}{\ln{\frac{\gamma_2}{\gamma_1}}}.
%\label{eq:AccelerationTime},
%\end{equation}

%which, together with Eq.~\ref{eq:RequiredAverageAccelGradient},
%leads to the final expression we were looking for, for the required average accelerating gradient,

%\begin{equation}
%G_{acc} = \frac{(\gamma_2-\gamma_1) E_0}{e c \tau_{acc}} = - \frac{E_0}{e c \tau_{\mu 0}} \frac{\ln{\frac{\gamma_2}{\gamma_1}}}{\ln{\frac{N_2}{N_1}}}.
%\label{eq:RequiredAverageAccelGradientFinal}
%\end{equation}

%\end{itemize} 

%\begin{flushleft}
%\interlinepenalty=10000
%\begin{thebibliography}{99}

%%%%%%%%%%%% Sensor refs %%%%%%%%%%%%%
%\bibitem{IMCC webpage}
%https://muoncollider.web.cern.ch/welcome-page-muon-collider-website.
%
%\bibitem{MAP}
%https://map.fnal.gov/.
%
%\bibitem{MICE}
%http://mice.iit.edu/.
%
%\bibitem{LEMMA}
%D.~Alesini et al., Positron driven muon source for a muon collider, arXiv:1905.05747 [physics.acc-ph].

%\end{thebibliography}
%\end{flushleft}


==> Chapters/99-DetectorPerformance_OldVersions/Author7.tex <==
\section{Detector Performance}

%\begin{flushleft}
%\blfootnote{
%This chapter should be cited as:
%The LHC machine and experiments, Eds. A.~Alici {\it et al.},
%DOI:~\href{https://doi.org/10.23730/CYRSP-2024-XXX.\thepage}{10.23730/CYRSP%-2024-XXX.\thepage},   in:
%Proceedings of the Joint Universities Accelerator School (JUAS): Courses %and exercises, E. M\'{e}tral (ed.),
%\\CERN Yellow Reports: School Proceedings, CERN-2024-XXX,
%DOI:~\href{https://doi.org/10.23730/CYRSP-2024-XXX}{10.23730/CYRSP-2024-XXX%},    p. \thepage.
%\\ \copyright\space CERN, 2021. Published by CERN under the
%\href{http://creativecommons.org/licenses/by/4.0/}{Creative Commons %Attribution 4.0 license}.
%}
%\end{flushleft}

\label{sec:Section7}

\noindent
The tables prepared by Fabian Batsch et al. and presented at the 1st meeting on HEMAC discussions (https://indico.cern.ch/event/1132527/) on 22/02/2022 can be found in Figs.~\ref{fig:Table1over2_MC-10T}~-~\ref{fig:Table2over2_MC-10T}~-~\ref{fig:Table1over2_MC-16T}~-~\ref{fig:Table2over2_MC-16T} below. They should be used as concerns the 3 RCS for the 3 TeV option. In fact, after the meeting it was decided to change the normal conducting magnets to 1.8T (instead of 1.5T). Going to 1.8T changes the length of the NC sections and thus decreases the filling factor, i.e. it gives more space for RF, etc. The updated tables can be found below in Figs.~\ref{fig:Table1over2_MC-2Tand16T}~-~\ref{fig:Table2over2_MC-2Tand16T}, which are the most up-to-date tables to be used.

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{Chapters/99-DetectorPerformance_OldVersions/Figures/Table1over2_MC-10T.png}
  \end{center}
\caption{Table 1/2 for 10T}
\label{fig:Table1over2_MC-10T}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{Chapters/99-DetectorPerformance_OldVersions/Figures/Table2over2_MC-10T.png}
  \end{center}
\caption{Table 2/2 for 10T}
\label{fig:Table2over2_MC-10T}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{Chapters/99-DetectorPerformance_OldVersions/Figures/Table1over2_MC-16T.png}
  \end{center}
\caption{Table 1/2 for 16T}
\label{fig:Table1over2_MC-16T}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{Chapters/99-DetectorPerformance_OldVersions/Figures/Table2over2_MC-16T.png}
  \end{center}
\caption{Table 2/2 for 16T}
\label{fig:Table2over2_MC-16T}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{Chapters/99-DetectorPerformance_OldVersions/Figures/Table1over2_MC-2Tand16T.png}
  \end{center}
\caption{Table 1/2 for 2T NC and 16T SC}
\label{fig:Table1over2_MC-2Tand16T}
\end{figure}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{Chapters/99-DetectorPerformance_OldVersions/Figures/Table2over2_MC-2Tand16T.png}
  \end{center}
\caption{Table 2/2 for 2T NC and 16T SC}
\label{fig:Table2over2_MC-2Tand16T}
\end{figure}

\clearpage

\begin{flushleft}
\interlinepenalty=10000
\begin{thebibliography}{99}

\bibitem{FabianBatschNoteApril2022}
F.~Batsch, Unit conversion for longitudinal emittances (https://cernbox.cern.ch/index.php/s/lvooRxgtE8pZQ4j).

\bibitem{emittancedef}
A.~Bogacz, \emph{Muon Acceleration -
Linac and RLA}, \url{https://indico.cern.ch/event/973753/contributions/4100198/attachments/2143992/3613246/Linac%20and%20RLA.pdf}, 2020 

% \bibitem{lhc_machine}
% O.S.~Brüning \textit{et al.} (Eds.),
% LHC design report, CERN-2004-003-V-1 (CERN, Geneva, 2004),
% \href{http://dx.doi.org/10.5170/CERN-2004-003-V-1} 
% {doi:10.5170/CERN-2004-003-V-1}  .

% \bibitem{lhc_dipole_train}
% A.~Verweij, Circuit performance at 6.5 TeV and beyond, LHC Performance Workshop, Chamonix,France, 2016,
% \href{https://indico.cern.ch/event/448109/contributions/1942054/attachments/1216245/1776253/2016_Chamonix_-_Verweij.pdf}{Indico}.

% \bibitem{machine_run2}
% J.~Wenninger,
% %LHC Status and Performance,
% \textit{PoS} \textbf{CHARGED2018} (2019) 001,
% \href{https://doi.org/10.22323/1.339.0001} 
% {doi:10.22323/1.339.0001} .


% \bibitem{ch3:Avoni:2018iuv}
% G.~Avoni \textit{et~al.},
% %M.~Bruschi, G.~Cabras, D.~Caforio, N.~Dehghanian, A.~Floderus, B.~Giacobbe, F.~Giannuzzi, F.~Giorgi, P.~Grafström, V.~Hedberg, F.~Lasagni Manghi, S.~Meneghini, J.~Pinfold, E.~Richards, C.~Sbarra, N.~Semprini Cesari, A.~Sbrizzi, R.~Soluk, G.~Ucchielli, S.~Valentinetti, O.~Viazlo, M.~Villa, C.~Vittori, R.~Vuillermet and A.~Zoccoli,
% %``The new LUCID-2 detector for luminosity measurement and monitoring in ATLAS,''
% \textit{JINST} \textbf{13} (2018) P07017,
% \href{https://doi.org/10.1088/1748-0221/13/07/P07017}
% {doi:10.1088/1748-0221/13/07/P07017}.
% %175 citations counted in INSPIRE as of 28 Jul 2020


% \bibitem{ch3:ATLAS-CONF-2019-021}
% ATLAS Collaboration,
% \href{https://cds.cern.ch/record/2677054}
% {Luminosity determination in $pp$ collisions at $\sqrt{s}=13$ TeV using the ATLAS detector at the LHC}, ATLAS-CONF-2019-021 (CERN Geneva, 2019).


\end{thebibliography}
\end{flushleft}

